Control Synthesis for Stability and Safety by Differential Complementarity Problem

This paper develops a novel control synthesis method for safe stabilization of control-affine systems as a Differential Complementarity Problem (DCP). Our design uses a control Lyapunov function (CLF) and a control barrier function (CBF) to define complementarity constraints in the DCP formulation to certify stability and safety, respectively. The CLF-CBF-DCP controller imposes stability as a soft constraint, which is automatically relaxed when the safety constraint is active, without the need for parameter tuning or optimization. We study the closed-loop system behavior with the CLF-CBF-DCP controller and identify conditions on the existence of local equilibria. Although in certain cases the controller yields undesirable local equilibria, those can be confined to a small subset of the safe set boundary by proper choice of the control parameters. Then, our method can avoid undesirable equilibria that CLF-CBF quadratic programming techniques encounter.

==> tex/Attachment.tex <==
\section{Getting ride of Assumption 1,2}
I'll record my findings about relaxing Assumption 1,2 here.

Since \eqref{DCP: CLC} and \eqref{DCP: CBC} shares the same solving method, I'll use \eqref{DCP: CLC} only here for simplification.

\subsubsection{Item 1} First we notice that \eqref{DCP: CLC} has the same solution to the following QP:
\begin{equation} \label{attach: min_norm_qp}
	\begin{aligned}
		\bfu &= \argmin_{\bfu \in \bbR^m} \, \frac{1}{2} \| \bfu \|_2^2  \\
		\mathrm{s.t.} \, &\, -\bfF_V(\bfx) - \mathcal{L}_{\bfG}V(\bfx) \cdot \bfu \geq 0.
	\end{aligned}
\end{equation}
for $\bfx \in \calC: \bfF_V(\bfx) \neq 0$.

Now, if we consider some $\bfx_s$ such that $\bfF_V(\bfx_s) = 0$ and $\mathcal{L}_{\bfG}V(\bfx_s) = \mathbf{0}$, the solution for the QP above is $\bfu(\bfx_s) = \mathbf{0}$, however, if we consider \eqref{DCP: CLC}, we would find that we have \eqref{DCP: CLC} satisfied for any $\bar{u}_l \in \bbR_{\geq 0}$. 

I think if we requires \eqref{DCP: CLC} to be hold only for $\bfx \in \calC: \bfF_V(\bfx) > 0$ and set $\bar{u}_l = 0$ for $\bfx \in \calC: \bfF_V(\bfx) \leq 0$, then the problem I mentioned above will be solved.
Otherwise we need to make an assumption that $\mathcal{L}_{\bfG}V(\bfx_s) \neq \mathbf{0} \forall \bfx \in \calC: \bfF_V(\bfx_s) = 0$.

\TODO{
I don't know if this expression: ``\eqref{DCP: CLC} is only need to be satisfied for $\bfx \in \calC: \bfF_V(\bfx) > 0$" is equivalent to saying that $\bar{u}_l = 0$ for $\bfx \in \calC: \bfF_V(\bfx) \leq 0$, if it is the case, then our notation would be much more simpler.
}

But anyway, by removing Assumption 1 and 2, at least we can't get the global closed-form expression as in \eqref{sol: bu_h_DBQ}.

Also, Pol mentioned in his paper that the solution to \eqref{attach: min_norm_qp} is Lipschitz. (Page 2, Column 2, After Definition 2)

\subsubsection{Item 2} If we take a look at \eqref{DCP: CBC}, things gets tricky, since we only requires that $\sup_{\bfu \in \bbR^m} [ \calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu ] \geq -\alpha_h(h(\bfx)), \ \forall \bfx \in \bbR^n$ NOT $\sup_{\bfu \in \bbR^m} [ \calL_{\bff} h(\bfx) + \mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_l\bar{u}_l + \calL_{\bfG} h(\bfx) \bfu ] \geq -\alpha_h(h(\bfx)), \ \forall \bfx \in \bbR^n$, so there might exists a $\bfx_s$ such that $\calL_{\bff} h(\bfx_s) + \alpha_h(h(\bfx_s)) \geq 0$ and $\calL_{\bfG} h(\bfx_s) = \mathbf{0}$ but $\calL_{\bff} h(\bfx_s) + \mathcal{L}_{\bfG}h(\bfx_s) \cdot \bfw_l(\bfx_s)\bar{u}_l(\bfx_s) < 0$, then \eqref{DCP: CBC} is infeasible.

\subsubsection{Item 3} Lipschitz continuity of $\bar{u}_l$ and $\bar{u}_h$ should be justified. In \cite{tan2021undesired} they said that: ``From \cite[Theorem 3]{xu2015robustness}, $\bfu(\bfx)$ as a solution of the CLF-CBF-QP formulation is locally Lipschitz continuous if $\calL_{\bfG}h(\bfx) \neq \mathbf{0} \forall \bfx \in \bbR^n$. In \cite{tan2021high}, this condition is further relaxed to requiring that the set of states at which $\calL_{\bfG}h(\bfx) = \mathbf{0}$ lies strictly inside the safety set"

\subsubsection{Item 4} Do we need $\bfA$ to satisfy Theorem 7.3.7 (c) even for the case where $\bfF_V(\bfx) < 0, \bfF_h(\bfx) + \mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_l\bar{u}_l > 0$. Since in this case we have $\bar{u}_l = 0, \bar{u}_h = 0$ no matter $\calL_{\bfG}V(\bfx)$ and $\calL_{\bfG}h(\bfx)$ equals zero or not due to the perpendicular constraint. \TODO{Also commented at the end of Section IV.}

\subsubsection{Item 5} Need to change some definitions and expressions in Local Equilibria Analysis section, but the impact to this section is small overall.

\subsubsection{Item 6} I'm copying the original sentence from \cite{tan2021undesired} since our definition of CLF and CBF are the same comparing to their paper: 
``Note that here we merely assume the existence of a CLF and a CBF, thus remove the assumptions that $\bfG(\bfx)$ is full rank as in \cite{reis2020control} or $\calL_{\bfG}h(\bfx) \neq \mathbf{0} \forall \bfx \in \bbR^n$ as in \cite{xu2015robustness}" 

This could be used as a backup plan if I can't find out anything in the end.

%\section{Existence of the solution to our ODE}
%\subsubsection{Failed Attempt 1}
%If the ultimate goal of requiring global Lipschitz for the R.H.S. of our ODE is to make sure that our solution $X(t)$ to it is finite for all $t >0$, then we could probably use this result I figured out:
%\begin{theorem}
%Consider closed-loop system $\dot{\bfx} = \bff_{cl}(\bfx) = \bff(\bfx) + \bfG(\bfx) \bfu$ with $\bfu$ given in \eqref{bfu: struct}, where $\bfw_l$ and $\bfw_h$ are given in \eqref{sel: bfw} with $\bar{u}_l$ and $\bar{u}_l$ takes the same value as in \eqref{sol: CBF-DCP}. If there exists a $l$-superlevel set of $V(\bfx)$: $\calV_l \coloneqq \{ \bfx \in \calC: V(\bfx) \leq l \}$ and a $b$-superlevel set of $h(\bfx)$: $\calH_b \coloneqq \{ \bfx \in \calC: h(\bfx) \leq b \}$ such that $\calV_l \subseteq \calH_b$ with $l,b >0$, then if we have the initial condition $\bfx_0$ for the closed-loop system satisfies $\bfx_0 \in \calV_l$, 
%\begin{proof}
%We only need to consider the case where we have $\bar{u}_h = 0$ since this is the only case we could have $\nabla h \bff_{cl}(\bfx) > 0$ (if $\bar{u}_h > 0$, then we must have $\nabla h \bff_{cl}(\bfx) + \alpha_h(h(\bfx)) = 0$, and due to the fact that $\alpha_h(h(\bfx)) \geq 0, \forall \bfx \in \calC$, we must have $\nabla h \bff_{cl}(\bfx) \leq 0, \forall \bfx \in \calC: \bar{u}_h > 0$). However, in this case we must satisfy $\nabla V \bff_{cl} < 0, \forall \bfx \in \calC \setminus \mathbf{0}$, 
%\end{proof}
%\end{theorem}

\subsubsection{Item 7:} I propose an alternative definition for CBF in order to keep our assumption on $\calL_{\bfG} h \neq \mathbf{0}, \forall \bfx \in \calD$

\begin{definition}\label{CBF_alt}
A continuously differentiable function $h(\bfx): \bbR^n \to \bbR$ is a \emph{control barrier function} (CBF) for system \eqref{dynamics: Sys_dynamics} defined on set $\calD$ with $\calC \subseteq \calD \subset \bbR^n$ if we have $\calL_{\bfG} h \neq \mathbf{0}$ for all $\bfx \in \calD$. 
\end{definition}
The set of safe control inputs at state $\bfx$ that renders the set $\calC$ forward invariant, corresponding to a valid CBF $h$, is \cite[Corollary 7]{xu2015robustness}:
%
\begin{equation}
	\nonumber
	K_{cbf}(\bfx) = \{ \bfu \in \bbR^m: \calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu \geq -\alpha_h(h(\bfx)) \}.
\end{equation}
%
where $\alpha_h: \bbR \to \bbR$ is an extended class $\calK$ function.


The follow theorem characterize under what conditions, the trajectory of \eqref{DCP: BQ-form} could converge to $\calQ$. \TODO{Something of this theorem could go wrong.}
\begin{theorem}
Assume $\bar{\calI} \cap \calS_i \neq \emptyset$, let $\calW$ be the largest neighborhood of $\bar{\calI} \cap \calS_i$ such that $\nabla f_h^{\top} \bfF_u(\bfx) > 0$ and $-\bfF_u(\bfx) \parallel^+ \bfG(\bfx) \bfw_p$. Then for any trajectories entering $\calQ$ with $\calQ \cap \calW \subset \calW$, the trajectory does not leave $Q$ for any $k$.
\begin{proof}
In $\calW$ we have $\nabla f_h^{\top} \bfG(\bfx) \bfw_p < 0$ due to the fact that $\bfF_u(\bfx)$ and $\bfG(\bfx) \bfw_p$ are linearly dependent and in the opposite direction. Also $\| \bfF_u(\bfx) \| < \bar{u}_h k \| \bfG(\bfx) \bfw_p \|, \forall \bfx \in \calW \cap \Omega \setminus \calQ \cap \calW \cap \Omega$. As a result, we have $\nabla f_h^{\top}[ \bfF_u(\bfx) + \bar{u}_h k \bfG(\bfx) \bfw_p ] = \nabla f_h^{\top} \dot{\bfx} < 0,  \forall \bfx \in \calW \cap \Omega \setminus \calQ \cap \calW \cap \Omega$ and the result follows.
\end{proof}
\end{theorem}

\TODO{%Finding a better expression for the theorem above. The idea for the following one is simple, but don't know whether $\calQ$ is connected or not, I think that is the reason why I prefer $\calS_i$. 

%If there exists a $\calQ_{k^*}$ such that
%$\calQ_{k_1} \subset \calQ_{k_2}, \forall k_1, k_2: 0 < k_1 < k_2 \leq k^*$ and  
%$\nabla f_h^{\top} \bfF_u(\bfx) > 0, -\bfF_u(\bfx) \parallel^+ \bfG(\bfx) \bfw_p, \forall \bfx \in \calQ_{k^*} \setminus \calQ_{\forall k: 0 < k < k^*}$, then it is non-removable from the trajectory of our system by increasing $k$.
%\begin{proof}
%We notice that for any $\bfx_q \in \calQ_{k^*}$, we could always find a $k < k^*$ such that $\bfx_q \notin \calQ_{k}$, however, we have $\nabla f_h^{\top} \bfG(\bfx) \bfw_p < 0$ due to the fact that $\bfF_u(\bfx)$ and $\bfG(\bfx) \bfw_p$ are linearly dependent and in the opposite direction for all $\bfx \in \calQ_{k^*} \setminus \calQ_{k}$. And we should notice that $\| \bfF_u(\bfx) \| < \bar{u}_h k \| \bfG(\bfx) \bfw_p \|, \forall \bfx \in \calQ_{k^*} \setminus \calQ_{k}$. As a result, we have $\nabla f_h^{\top}[ \bfF_u(\bfx) + \bar{u}_h k \bfG(\bfx) \bfw_p ] = \nabla f_h^{\top} \dot{\bfx} < 0,  \forall \bfx \in \calQ_{k^*} \setminus \calQ_{k}$ and the result follows.
%\end{proof}
I'm trying to give some detailed explanation here.

If the trajectory intersects set $\calS \coloneqq \{ \bfx \in \partial \calC: f_h(\bfx) = 0 \}$, it is equivalent to consider a system starts with $\bfx_0 \in \calS$. 

Now assume the trajectory intersects $\calS$, so with out loss of generality, we could consider system starts with $\bfx_0 \in \calS$ and use $\bfX(t,\bfx_0)$ to denoted the unique solution to our system (CLF-CBF-DCP with $\bfw_l$ and $\bfw_h$ given in \eqref{sel: bfw}). We should notice that $f_h(\bfx) = 0$ implies $\bar{u}_h = 0$ (but the converse not holds outside $\partial \calC$), so we have $\dot{\bfx} = \bfF_u(\bfx)$ for all $\bfx \in \calS$.
We consider the following scenarios:
\subsubsection{Scenarios 1} $\bfx_0 \in \{ \bfx \in \calS: \nabla f_h^{\top}(\bfx) \bfF_u(\bfx) = 0 \}$

In this case we could have 1) $\nabla f_h^{\top}(\bfX(t_1)) \bfF_u(\bfX(t_1)) > 0$ at $t_1 > 0$; 2) $\nabla f_h^{\top}(\bfX(t_2)) \bfF_u(\bfX(t_2)) < 0$ at $t_2 > 0$; 3) $\nabla f_h^{\top}(\bfX(t)) \bfF_u(\bfX(t)) = 0$ for all $t > 0$.
We will discuss 1) and 2) in later scenarios, but if we have 3), which indicates that $f_h(\bfX(t)) = 0$ for all $t > 0$, then we will never separate from $\partial \calC$. Since $f_h(\bfX(t)) = 0$ implies $\nabla h^{\top}(\bfX(t)) \bfF_u\bfX(t) = 0$ and thus $h(\bfX(t)) = 0$ for all $t > 0$.

\subsubsection{Scenarios 2} $\bfx_0 \in \{ \bfx \in \calS: \nabla f_h^{\top}(\bfx) \bfF_u(\bfx) > 0 \}$

In this case we will immediately have $f_h(\bfX(t)) > 0$ for arbitrary small $t > 0$, thus we will not separate from $\partial \calC$ at points belongs to $\bar{\calI} \coloneqq \{ \bfx \in \calS: \nabla f_h^{\top}(\bfx) \bfF_u(\bfx) > 0 \}$.

\subsubsection{Scenarios 3} $\bfx_0 \in \{ \bfx \in \calS: \nabla f_h^{\top}(\bfx) \bfF_u(\bfx) < 0 \}$

In this case we will immediately have $f_h(\bfX(t)) < 0$ for arbitrary small $t > 0$, thus we will separate from $\partial \calC$ at points belongs to $\bfx_0 \in \{ \bfx \in \calS: \nabla f_h^{\top}(\bfx) \bfF_u(\bfx) < 0 \}$.

Now we no longer assume $\bfx_0 \in \calS$, instead we assume $\bfx_0 \in \calX_a \coloneqq \{ \bfx \in \partial \calC: f_h(\bfx) > 0 \}$ and study the problem: will we have $\bfX(t) \in \calS$ for some $t > 0$? However, we could not reach every points belongs to $\calS$ from $\calX_a$, only points in $\calS_c \coloneqq \{ \bfx \in \calS: \calB_{\epsilon}(\bfx) \cap \calX_a \neq \emptyset, \forall \epsilon > 0 \}$ could be reached from $\calX_a$. Also, during the reaching process, we will run into some issue if we have $\bfF_u(\bfx)$ and $\bfG(\bfx) \bfw_p$ linearly dependent, so we define the following set $\calS_d \coloneqq \{ \bfx \in \calS_c: \bfF_u(\bfx) \parallel \bfG(\bfx) \bfw_p \vee -\bfF_u(\bfx) \parallel \bfG(\bfx) \bfw_p \}$ (I want to use $\parallel$ to denote linearly dependent and in the same direction to save some space, so I use the $\vee$ symbol here). Now considering the following two cases:

\subsubsection{Case 1} We want to reach some points belongs to $\calS_d \setminus \calS_i$ ($\bfF_u(\bfx)$ and $\bfG(\bfx) \bfw_p$ in same direction).

For points belongs to $\calS_d \setminus \calS_i$ such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) = 0$, we don't know if we could reach them.

For points belongs to $\calS_d \setminus \calS_i$ such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) < 0$, we could reach them if we enters a small ball around those points such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) < 0$ and $\bfF_u(\bfx), \bfG(\bfx) \bfw_p$ linearly dependent for every points in these small balls.

For points belongs to $\calS_d \setminus \calS_i$ such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) > 0$, we could not reach them since there exists a small ball around those points such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) > 0$ and $\bfF_u(\bfx), \bfG(\bfx) \bfw_p$ linearly dependent for every points in these small balls.

\subsubsection{Case 2} We want to reach some points belongs to $\calS_d \cap \calS_i$ ($\bfF_u(\bfx)$ and $\bfG(\bfx) \bfw_p$ in opposite direction). 

For points belongs to $\calS_d \cap \calS_i$ such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) = 0$, we don't know if we could reach them.

For points belongs to $\calS_d \cap \calS_i$ such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) < 0$, we could not reach them since there exists a small ball around those points such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) < 0$ and $\bfF_u(\bfx), \bfG(\bfx) \bfw_p$ linearly dependent for every points in these small balls, then we have $\nabla f_h^{\top}(\bfx) \bfG(\bfx) \bfw_p > 0$. Assume now we have $\bfx_0 \in \calX_a$ belongs to such balls, then we can always choose $k$ sufficient small such that $\bfx_0 \notin \calQ$, then we will have $f_h(\bfX(t)) > f_h(\bfX(t_0 = 0))$ at least for some small $t$. And if we choose $k=0$ for such $\bfx_0$, then we will reach $\bfX(t) \in \calS_d \cap \calS_i$ such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) < 0$ for some $t$.

For points belongs to $\calS_d \cap \calS_i$ such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) > 0$, we could not reach them since there exists a small ball around those points such that $\nabla f_h^{\top}(\bfx) \bfF_u(\bfx) > 0$ and $\bfF_u(\bfx), \bfG(\bfx) \bfw_p$ linearly dependent for every points in these small balls, then we have $\nabla f_h^{\top}(\bfx) \bfG(\bfx) \bfw_p < 0$. Assume now we have $\bfx_0 \in \calX_a$ belongs to such balls, then we can always choose $k$ sufficient small such that $\bfx_0 \notin \calQ$, then we will have $f_h(\bfX(t)) < f_h(\bfX(t_0 = 0))$ at for all $t < t^*$ where $t^* = \argmin_t \bfX(t) \in \calQ$. Hence, no matter how we increase $k$ we will always run into corresponding $\calQ$.
}

==> tex/Evaluation_Alt.tex <==

%stabilization with two different obstacle types.

\section{Evaluation} 

\MODI{We compare our \emph{CLF-CBF DCP} with the \emph{relative CLF-CBF QP} introduced in \cite{tan2021undesired}, which computes a relative perturbation to a nominal stabilizing controller, the \emph{adaptive CLF-CBF QP} introduced in \cite{pol2022roa}, which uses a CBF QP with an adaptive CLF penalty, and the \emph{Lyapunov shaping} introduced in \cite{reis2020control}, which CLF is subject to rotation controlled by an extra CBF like constraint.} 
To make a clear comparison, we use the same planar fully actuated system in our evaluation, $\dot{\bfx} = \bfx + \bfu$ with $\bfx,\bfu \in \bbR^2$. We consider two scenarios.
%
\begin{itemize}[align=left,leftmargin=1em]
    \item[Case 1]: \emph{Convex obstacle with poorly constructed CLF}: We use CBF $h(\bfx) = x_1^2 + (x_2 - 4)^2 -4$ with $\alpha_h(h) = h$ and CLF $V(\bfx) = \frac{1}{2} (6x_1^2 + x_2^2)$ with $\alpha_l(V) = V$.
    %Results are shown in Fig.~\ref{fig: cir_6_ck}
    %\NA{This should be moved and discussed later. We are describing the setup now, not the results.}.
    
    %\item[Case 2]: \emph{Concave obstacle with well constructed CLF}: We use CBF $h(\bfx) = \big( (x_1-2)^2+(x_2-3)^2 \big)\big( (x_1+2)^2+(x_2-3)^2 \big) - 2.1^4$ with $\alpha_h(h) = h$ and CLF $V(\bfx) = \frac{1}{2} (x_1^2 + x_2^2)$ with $\alpha_l(V) = V$. 
    %Results are shown in Fig.~\ref{fig: con_ck}\NA{This should be moved and discussed later. We are describing the setup now, not the results.}.
    \MODI{\item[Case 2]: \emph{Concave obstacle with non-radial CLF}: We use CBF $h(\bfx) = \big( (x_1-2)^2+(x_2-3)^2 \big)\big( (x_1+2)^2+(x_2-3)^2 \big) - 2.1^4$ with $\alpha_h(h) = h$ and CLF $V(\bfx) = \frac{1}{2} (x_1^2 + 2x_2^2)$ with $\alpha_l(V) = V$. }
\end{itemize}


%on the ability to avoid local equilibria. 
%We use the following two-dimensional system: $\dot{\bfx} = \bfx + \bfI_2 \bfu$ with $\bfx = [x_1,x_2]^{\top}$, i.e., $\bff(\bfx) = \bfx$, $\bfG(\bfx) = \bfI_2$.
%We test our proposed CLF-CBF DCP with two distinct scenarios: \\
%\NA{Instead of using bold it might be better to use bullets. The paragraph looks very crammed now. Never sacrifice readability for space gains.}
% \textit{Case 1 (Circular obstacle with badly constructed CLF):} In this case we have our CBF given by: $h(\bfx) = x_1^2 + (x_2 - 4)^2 -4$ with $\alpha_h(h) = h(\bfx)$ and CLF given by: $V(\bfx) = \frac{1}{2} (6x_1^2 + x_2^2)$ with $\alpha_l(V) = V(\bfx)$. Results are shown in Fig.~\ref{fig: cir_6_ck}.
% %
% \textit{Case 2 (Concave obstacle with decently constructed CLF):} In this case we have our CBF given by: $h(\bfx) = \big( (x_1-2)^2+(x_2-3)^2 \big)\big( (x_1+2)^2+(x_2-3)^2 \big) - 2.1^4$ with $\alpha_h(h) = h(\bfx)$ and CLF given by: $V(\bfx) = \frac{1}{2} (x_1^2 + x_2^2)$ with $\alpha_l(V) = V(\bfx)$. Results are shown in Fig.~\ref{fig: con_ck}.




\begin{figure}[t]
	\centering
	\includegraphics[width=.84\linewidth,trim=12mm 8mm 15mm 12mm, clip]{Fig2wRef9.pdf}
	\caption{\MODI{Comparison of CLF-CBF-DCP controller to the relative CLF-CBF-QP controller by \cite{tan2021undesired}, the adaptive CLF-CBF-QP controller by \cite{pol2022roa} and the Lyapunov shaping by \cite{reis2020control} with a circular obstacle (\textbf{\textcolor{green}{green}}) and various initial conditions (\textbf{black} dots). Both QP-based methods converge to an undesired local equilibrium $(0,6)$ on the safe set boundary with initial conditions satisfying $x_2(0) > 4$. While Lyapunov shaping converge to undesired local equilibria inside the safe set.
	%This is due to the chosen CLF, which admits a large region of attraction for $(0,6)$ for the QP-based methods. 
	In contrast, the CLF-CBF-DCP controller achieves both safety and stability at the origin.}}
	\label{fig: cir_6_ck}
\end{figure}

% \begin{figure}[t]
% 	\centering
	
% \end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth,trim=5mm 4mm 5mm 8mm, clip]{Fig5wRef9.pdf}
	\caption{\MODI{Comparison results with a concave obstacle (\textbf{\textcolor{green}{green}}) using non-radial CLF. Both the relative CLF-CBF-QP and the adaptive CLF-CBF-QP controllers get stuck at a boundary equilibrium $(0,3.65)$ under initial conditions $(\pm0.5, 4)$ and $(1,5)$, while Lyapunov shaping controller get stuck at different boundary local equilibria under initial conditions $(\pm0.5, 4)$. In addition, Lyapunov shaping get stuck at interior local equilibria for the rest initial conditions. In contrast, the CLF-CBF-DCP controller achieves both safety and asymptotic stability at the origin.}}\label{fig: con_ck}
	~\\
    \subcaptionbox{$k = 14.6$ at the \textit{plus} point\label{fig: k_test_fail}}{\includegraphics[width=0.5\linewidth,trim=5mm 2mm 5mm 8mm, clip]{Fig4FwRef9.pdf}}%
    \hfill%
    \subcaptionbox{$k = 15$ at the \textit{plus} point\label{fig: k_test_succ}}{\includegraphics[width=0.5\linewidth,trim=5mm 2mm 5mm 8mm, clip]{Fig4SwRef9.pdf}}%
    \caption{\MODI{The CLF-CBF-DCP controller with different choices of $k$ initialized at the \textbf{black} plus point $(-5,4)$. Fig.~\ref{fig: k_test_fail} shows that if $k$ is not sufficiently large, a local equilibrium exists on the obstacle boundary at the \textbf{\textcolor{orange}{orange}} star point. Fig.~\ref{fig: k_test_succ} shows that this equilibrium can be eliminated by increasing $k$. }}
    \label{cir: k_test}
\end{figure}


In each case, since $\bfG(\bfx) = \bfI_2$, $\bfw_p(\bfx)$ satisfying \eqref{wp-cond} can be chosen as $\nabla h(\bfx)^\top \bfw_p(\bfx) = 0$ with $\| \bfw_p(\bfx) \|_2 = 1$. There are two choices for such $\bfw_p$ with opposite signs. In the simulations, for some interesting initial conditions, we show the closed-loop CLF-CBF-DCP trajectory for both choices.


%From two choices for such $\bfw_p$ with opposite signs, we show the results under both choices for some initial conditions and under one picked choice for the other initial conditions.   
%\TODO{There are two choices for such $\bfw_p$ with opposite signs. We simulate both cases under several initial conditions, and as a result, both cases are observed to achieve the safety and stability. However, in the simulation figure, we show the both cases only under the initial condition $x_1(0) =0 $, while the simulation under the other initial conditions are shown only for one choice of the sign which does not go beyond the region of the environment.}\NA{This discussion is useless and wastes a lot of space.} 
%However, both $\bfw_p$ and $-\bfw_p$ satisfies our criteria, we manually select one of them for every initial conditions except ($0,9$), ($0,6$) in Case 1 and ($0,5.3$), ($0,3.65$) in Case 2, where we use $\pm \bfw_p$.

%The trajectories generated by the three controllers for Cases 1 and 2 are shown in Fig.~\ref{fig: cir_6_ck} and Fig.~\ref{fig: con_ck}, respectively. 
\MODI{The trajectories generated by the four controllers for Cases 1 and 2 are shown in Fig.~\ref{fig: cir_6_ck} and \ref{fig: con_ck}, respectively.
Both QP-based and Lyapunov shaping methods converge to undesirable equilibria for some initial conditions, depending on the shape of the safe set. In these cases, our CLF-CBF-DPC controller achieves both safety and asymptotic stability at the origin for all tested initial conditions. The diamond and square points in the figures depict the locations of the set $\calS$, which is determined by $\bfw_p(\bfx)$. If the system trajectory passes through the \emph{diamond} point, then only the \emph{square} point belongs to $\calS$, and vice versa. Thus, in these examples the closed-loop trajectory does not pass through the set $\calS$.}

%$\bfw_p(\bfx)$ makes the trajectory passes the \textit{diamond} (\textit{square}) point, then we only have the \textit{square} (\textit{diamond}) point belongs to $\calS$, thereby the trajectory does not pass through the equilibria set.
%\begin{comment}
%once the sign of $\bfw_p(\bfx)$ is chosen, the trajectory passes through the set $\calS$ determined by the other sign of $\bfw_p$\NA{I am not sure what this means}, thereby the trajectory does not pass through the equilibria set. 
%\end{comment}
Fig.~\ref{cir: k_test} shows the effect of the term $k$ in \eqref{sel: bfw} on the DCP controller. For small values of $k$ in Fig.~\ref{cir: k_test}(a), the trajectory gets stuck at an undesired local equilibrium, while for larger $k$, shown in Fig.~\ref{cir: k_test}(b), it converges to the origin. %Interestingly, we observe that $\inf_{\bfx \in \calX} \bar{u}_h = 0$ in this scenario, which lets us conjecture that even when $\inf_{\bfx \in \calX} \bar{u}_h = 0$, for sufficiently large $k>0$ and depending on $\bfw_p(\bfx)$, the closed-loop trajectory may avoid the undesired equilibria in $\calQ$ and stabilize the system at the origin.

\MODI{Without any further conditions, both CLF-CBF DCP and relative CLF-CBF QP introduce no local equilibria in $\textrm{Int}(\calC)$. While adaptive CLF-CBF QP needs to satisfy \cite[Corollary 5.4]{pol2022roa} to remove local equilibria in $\textrm{Int}(\calC)$, and as Fig.~\ref{fig: cir_6_ck}, \ref{fig: con_ck} shows, Lyapunov shaping fails to address local equilibria in $\textrm{Int}(\calC)$. On the other hand, relative CLF-CBF QP will stuck at local equilibria on $\partial \calC$ if it satisfies $L_{\mathfrak{g}}h \neq \mathbf{0}$ \cite[Theorem~3.(3)]{tan2021undesired} and so as adaptive CLF-CBF QP if \cite[Remark 2]{pol2022roa} holds. While Lyapunov shaping could only address local equilibria on $\partial \calC$ caused by collinearity among vectors $f(x)$, $G(x)\nabla V(x,Q)$ and $G(x)\nabla h(x)$, as demonstrated through Fig.~\ref{fig: cir_6_ck}.}

%\NA{We do not say anything about the other methods in the discussion. Did we choose their parameters well? Do they always get stuck? Why? What else do we observe about their performance? How does our controller differ from theirs given that both have closed-forms -- is there a particular term in the closed form expression that might contribute to the observed behavior?}







%, though $\inf \bar{u}_h = 0$ in this scenario. This observation lets us conjecture that, even if $\inf_{\bfx \in \calX} \bar{u}_h = 0$, for sufficiently large $k>0$ and a chosen $\bfw_p$, the closed-loop trajectory does not arrive at the undesired local equilibria, thereby the stabilization at the origin is achieved. 
%Figuring out this property from theoretical perspective is our future work\NA{This conflicts with what we say in the conclusion. Perhaps move this to the conclusion.}. 

%While our theoretical results only ensures that there are equilibria only in $\calQ$ for 
% While, 
% both CLF-CBF DCP and relative CLF-CBF QP introduce no local equilibria in $\textrm{Int}(\calC)$ while adaptive CLF-CBF QP needs to satisfy \cite[Corollary 5.4]{pol2022roa} to remove local equilibria in $\textrm{Int}(\calC)$. 
% According to Proposition~\ref{local_equilibria}, we could always find a constant $k$ such that $\calQ$ will not appear in our trajectories unless we are converging to $\calS$. While relative CLF-CBF QP gets stuck at a local equilibria on $\partial \calC$ if it satisfies \cite[Proposition 3]{tan2021undesired}, so as adaptive CLF-CBF QP if \cite[Remark 2]{pol2022roa} holds.
%Take Fig.~\ref{fig: cir_6_ck} for example, if $\bfw_p$ makes our system separates from $\partial \calC$ at the \textit{diamond} (\textit{square}) point, then we only have the \textit{square} (\textit{diamond}) point belongs to $\calS$. As a result, there always exists a constant $k$ restricting $\calQ$ to a small neighborhood of the \textit{square} (\textit{diamond}) point to make it out of the trajectories of our systems. In Fig.~\ref{cir: k_test} we give an example considering the case where we have $k$ not large enough. 



% %\NA{It is standard to use Fig.~\ref{fig: cir_6_ck} instead of Figure~\ref{fig: cir_6_ck}.}
% \begin{comment}
% %be noted that $\bar{\calI} = \emptyset$ for both cases since we only have $f_h(\bfx) = 0$ at the \textit{diamond} and \textit{square} points and we could separate from $\partial \calC$ at both of them with particular choice of $\bfw_p$, as a result, 
% %since for this particular choice of $\bfw_p$, we will never reach the \textit{square} point unless our system hits right on it. Now assume we have a sufficient large $k$ with same $\bfw_p$, as we pointed our in \ref{k: constant}, local equilibria $\bfx^*$ exists and we could push it arbitrary close to the \textit{square} point by increasing $k$. However, even if we start our system with $\bfx_0 = \bfx^*$, we still could push $\bfx^*$ even closer to the \textit{square} point by increasing $k$, and as a result, push $\bfx^*$ out of our desired trajectory (trajectory generated by $\dot{\bfx} = \bfG(\bfx)\bfw_p$ with $\bfx_0 = \bfx^*$ solely). Also, I need to point out that we could play this trick because both the \textit{diamond} point and the \textit{square} point are NOT belongs to $\bar{\calI}$, since in this case we will push $\bfx^*$ further into our desired trajectory. 

% % \begin{figure*}[t]
% % 	\begin{subfigure}{\columnwidth}
% % 		\centering
% % 		\includegraphics[width=\columnwidth]{cir_test_fail.pdf}
% % 		\caption{$k = 14.6$ at the \textit{plus} point}
% % 		\label{fig: k_test_fail}
% % 	\end{subfigure}%
% % 	\begin{subfigure}{\columnwidth}
% % 		\centering
% % 		\includegraphics[width=\columnwidth]{cir_test_succ.pdf}
% % 		\caption{$k = 15$ at the \textit{plus} point}
% % 		\label{fig: k_test_succ}
% % 	\end{subfigure}
% % 	\caption{CLF-CBF-DCP with different choice of $k$ starting at the \textit{plus} point ($-5,4$) tempting to separates at the \textit{diamond} point from the obstacle boundary. Fig.~\ref{fig: k_test_fail} shows that if $k$ is not sufficient large, we will run into a local equilibrium marked as the \textit{star} point on the obstacle boundary and Fig.~\ref{fig: k_test_succ} shows that this equilibrium could be easily addressed by increasing $k$. }
% % 	\label{cir: k_test}
% % \end{figure*}

% %\NA{This subsection should be integrated in the Simulations section} 
% %Now we distinguish the difference between our CLF-CBF-DCP with relative CLF-CBF-QP introduced in \cite{tan2021undesired} and adaptive CLF-CBF-QP introduced in \cite{pol2022roa} from the theoretical perspective.
% %Also, relative CLF-CBF-QP will stuck at local equilibria on $\partial \calC$ if it satisfies \cite[Proposition 3]{tan2021undesired} and so as adaptive CLF-CBF-QP if \cite[Remark 2]{pol2022roa} holds. Although our CLF-CBF-DCP formulation will always admit some local equilibria on $\partial \calC$ satisfying \eqref{equilibria-cond} when there exists no finite $k$ satisfying \eqref{criteria: k}, we can restrict them to a particular set $\calQ$ by using an alternative approach \eqref{criteria: relax_k} for determining $k$. Nevertheless, we can even remove the set of the local equilibria $\calQ$ from the trajectory by shrinking the size of $\calQ$ via increasing $k$ (i.e. decreasing $\nu$). 
% \end{comment}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\section{Conclusion} 
We formulated control synthesis with CLF stability and CBF safety constraints as a DCP. We proved that the CLF-CBF-DCP control law is Lipschitz continuous and characterized the closed-loop system equilibria. We demonstrated how an extra forcing term may eliminate undesired equilibria that CLF-CBF-QP techniques encounter. %Future work will explore input constraints, multiple and higher-order CBFs, as well as applications to autonomous robot systems.

% extensions of the proposed method to 

%We have proposed a novel control synthesis method for safety and stability based on differential complementary problem and constructed the CLF-CBF-DCP controller. We prove that the closed-loop dynamics of CLF-CBF DCP are Lipschitz continuous and characterized the closed-loop system equilibria. Under suitable assumptions, we demonstrated how to construct the extra forcing term to eliminate local equilibria. Future work will explore the extension of the proposed method to input constraints, multiple and higher-order CBFs.


\begin{comment}
Possible future research topics. 

First, CLF-CBF-DCP based model predictive control (MPC), since for now we are making decisions based on information provided by the current state. I tried to figure our the conditions under which we will converge to $\calQ$, but for now, I could only find the condition for 2-D case, if we want to consider a higher dimensional system, then the information provided by the current state is not enough, we need to consider the trajectory under the current control law. The difficult part for higher dimensional case is that we need to guarantee the forward invariant of the following set $\calH \coloneqq \{ \bfx \in \partial \calC: -\bfF_u(\bfx) \parallel \bfG(\bfx)\bfw_p(\bfx), \nabla \bar{u}_h^{\top} \bfF_u(\bfx) < 0, 0 < \bar{u}_h < \omega \}$, where $\omega$ is a constant. In our case, if we have $\calQ \cap \calH \subset \calH$, then for every point belongs to $\calH \setminus \calQ$, we could guarantee $\nabla \bar{u}_h^{\top} \dot{\bfx} < 0$, thus the $0 < \bar{u}_h < \omega$ would not be a problem. The hard part lies in how to find a boundary condition to ensure the $-\bfF_u(\bfx) \parallel \bfG(\bfx)\bfw_p(\bfx)$ constraint is forward invariant. This problem could be easily addressed through MPC since we only need to ensure the trajectory generated by $\dot{\bfx} = \bfG(\bfx) \bfw_p(\bfx)$ with $\bfx_0 \in \calH \setminus \calQ$ stays in $\calH$ for $0 < t < t^*$, with %t^*% the smallest time such that $\bar{u}_h = 0$.
\end{comment}

==> tex/Old_approach.tex <==
\section{CBF-DCP Formulation} This section shows how to combine CLF ($V$) and CBF ($h$) as a DCP. Consider control affine nonlinear dynamic system \eqref{dynamics: Sys_dynamics} and we parameterize the control input $\bfu$ as follows:
%
\begin{equation}
	\label{bfu: struct}
	\bfu = \bfw_l\bar{u}_l + \bfw_h\bar{u}_h,
\end{equation}
%
where we have locally Lipschitz $\bfw_l, \bfw_h \in \bbR^m$ with $\bar{u}_l, \bar{u}_h \in \bbR$.
We propose the following CBF-DCP:
%
\begin{subequations}
	\label{DCP: BQ-form}
	\begin{align}
		&\dot{\bfx} = \bff(\bfx) + \bfG(\bfx)[\bfw_l\bar{u}_l + \bfw_h\bar{u}_h], \ \forall \bfx \in \calD \nonumber \\
		\mathrm{s.t.} \, \, & 0 \leq \bar{u}_l \perp -\bfF_V(\bfx) - \mathcal{L}_{\bfG}V(\bfx) \cdot \bfw_l\bar{u}_l \geq 0, \label{DCP: CLC} \\
		& 0 \leq \bar{u}_h \perp \bfF_h(\bfx) + \mathcal{L}_{\bfG}h(\bfx) \cdot [\bfw_l\bar{u}_l + \bfw_h\bar{u}_h] \geq 0 \label{DCP: CBC}
	\end{align}
\end{subequations}
%
where $\bfF_V(\bfx) = \mathcal{L}_{\bff}V(\bfx) + \alpha_l(V)$, $\bfF_h(\bfx) = \mathcal{L}_{\bff}h(\bfx) + \alpha_h(h)$. In order to guarantee the uniqueness of solutions to \eqref{DCP: CLC}-\eqref{DCP: CBC}, we need to have the following constraints on design parameters $\bfw_l$ and $\bfw_h$: $-\mathcal{L}_{\bfG}V(\bfx) \cdot \bfw_l > 0$ and $\mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_h > 0, \ \forall \bfx \in \calD$. A \textit{naive choice} of $\bfw_l$ and $\bfw_h$ would be $-\mathcal{L}_{\bfG}V(\bfx)^{\top}$ and $\mathcal{L}_{\bfG}h(\bfx)^{\top}$ respectively.
The solution of the CBF-DCP above is characterized by the following theorem.
%
\begin{theorem} \label{trem: sol_DCP-BQ}
	The solution of \eqref{DCP: CLC}-\eqref{DCP: CBC} is unique and takes the following closed-form expression:
	%
	\begin{equation} 
		\label{sol: DCP-BQ}
		\begin{aligned}
			&\bar{u}_l = \left( -\frac{\bfF_V(\bfx)}{\mathcal{L}_{\bfG}V(\bfx) \cdot \bfw_l} \right)_+, \\
			&\bar{u}_h = \left(-\frac{\bfF_h(\bfx) + \mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_l \bar{u}_l }{\mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_h}\right)_+
		\end{aligned}
	\end{equation}
	%
	where $(\cdot)_+$ denotes $\max(\cdot,0)$.
	\begin{proof} We notice that
		$\left[ \begin{matrix}
			 -\mathcal{L}_{\bfG}V(\bfx) \cdot \bfw_l & 0\\
			\mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_l & \mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_h
		\end{matrix} \right]$
	is a $P$-matrix, thus the uniqueness result follows directly from Proposition~\ref{prop: DCP_uniqueness}. Also, once we obtain the closed-form expression of $\bar{u}_l$ from \eqref{DCP: CLC}, we could simplify \eqref{DCP: CBC} by substituting $\bar{u}_l$ with its closed-from expression and \eqref{DCP: CBC} will have the same structure as \eqref{DCP: CLC}. Thus we only consider \eqref{DCP: CLC} since \eqref{DCP: CBC} could be solved using exactly the same procedure: If we have $\bar{u}_l = 0$, then $-\bfF_V(\bfx) \geq 0$ should holds. If we have $\bar{u}_l > 0$, then $-\bfF_V(\bfx) - \mathcal{L}_{\bfG}V(\bfx) \cdot \bfw_l\bar{u}_l = 0$ should holds, and we solve the equation above to obtain $\bar{u}_l = -\frac{\bfF_V(\bfx)}{\mathcal{L}_{\bfG}V(\bfx) \cdot \bfw_l}$. However since we require $\bar{u}_l > 0$, $-\bfF_V(\bfx) < 0$ should also holds. Above all, we conclude that $\bar{u}_l = ( -\frac{\bfF_V(\bfx)}{\mathcal{L}_{\bfG}V(\bfx) \cdot \bfw_l} )_+$. 
	\end{proof}
\end{theorem}
%\YY{I will revisit the proof part of this theorem later, maybe in the fashion of evaluating KKT conditions. Depending on how much space left.}
\begin{remark}
	One might notice that our CBF-DCP formulation \eqref{DCP: BQ-form} is based on the CBF-QP formulation \eqref{controller: CBF-QP} since in both cases, \TODO{the stabilizing control input only serves as an reference control input}. However, instead of using a given stabilizing control input $\bfr(\bfx) \in K_{clf}(\bfx)$, the stabilizing control input in our formulation \eqref{DCP: BQ-form} is obtained through \eqref{DCP: CLC}. 
\end{remark} 
%\YY{This remark is unclear with "stabilizing control input is independent of..."}
By making the \textit{naive choice} of $\bfw_l$ and $\bfw_h$, control input $\bfu$ generated by \eqref{DCP: CLC}-\eqref{DCP: CBC} is given by the following equation: 
%
\scriptsize
\begin{equation}\label{sol: CBF-DCP}
	\bfu = -( \frac{\bfF_V(\bfx)}{\| \mathcal{L}_{\bfG}V(\bfx) \|_2^2} )_+ \mathcal{L}_{\bfG}V(\bfx)^{\top} + (-\frac{\nabla h(\bfx) \cdot \ \bfe(\bfx) + \alpha_h(h)}{\| \calL_{\bfG} h(\bfx) \|_2^2})_+ \calL_{\bfG} h(\bfx)^{\top}
\end{equation}
\normalsize
%
with $\bfe(\bfx)$ defined in Proposition~\ref{sol: QP}.
\subsection{Connecting DCP and QP Based Methods}
\TODO{In this section, we abuse the use of terminology equivalent. In our paper, when we say that the two systems are equivalent or attain equivalency, we mean that they receive the same control input at the same state.}
We first notice that our CBF-DCP is equivalent to CBF-QP if we take the \textit{naive choice} of $\bfw_l, \bfw_h$ and set $\bfr(\bfx) = -( \frac{\bfF_V(\bfx)}{\| \mathcal{L}_{\bfG}V(\bfx) \|_2^2} )_+ \mathcal{L}_{\bfG}V(\bfx)^{\top}$ in \eqref{controller: CBF-QP}. However, if we want to use a given reference stabilizing control input $\bfr(\bfx)$ in CBF-QP other than the solution of \eqref{DCP: CLC}, we need to construct a different DCP to attain equivalency as the following proposition shows.
\begin{proposition}\label{DCP: BQ-Equi} The following DCP system is equivalent to the CBF-QP formulation:
	%
	\begin{subequations}
		\label{DCP: CBF-QP_equi}
		\begin{align}
			&\dot{\bfx} = \bff(\bfx) + \bfG(\bfx)[\bfr(\bfx) + \bfw_h\bar{u}_h], \nonumber \\
			\mathrm{s.t.} \, \, 
			& 0 \leq \bar{u}_h \perp \bfF_h(\bfx) + \mathcal{L}_{\bfG}h(\bfx) \cdot [\bfr(\bfx) + \bfw_h\bar{u}_h] \geq 0 \label{CBC: DBQ}
		\end{align}
	\end{subequations}
	%
	where $\bfw_h = \mathcal{L}_{\bfG}h(\bfx)^{\top}$.
	\begin{proof}
		The solution to \eqref{CBC: DBQ} is easily obtained as follows:
		\begin{equation}
			\label{sol: bu_h_DBQ}
			\bar{u}_h = (-\frac{\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx)\bfr(\bfx) + \alpha_h(h)}{\| \calL_{\bfG} h(\bfx) \|_2^2})_+
		\end{equation}
		and we have $\bfu = \bfr(\bfx) + \bfw_h\bar{u}_h = \bfr(\bfx) + \bar{u}_h \calL_{\bfG} h(\bfx)^{\top}$, which is the same as the solution for CBF-QP formulation as \eqref{sol: CBF-QP} shows.
	\end{proof}
\end{proposition}
In addition to that , if we consider the following CLF-CBF-QP:
%
\begin{equation}\label{controller: CLF-CBF-QP}
	\begin{aligned}
		\bfu(\bfx) = & \argmin_{(\bfu, \delta) \in \bbR^{m+1}} \frac{1}{2} || \bfu ||_2^2 + \frac{1}{2} p \delta^2 \\
		\mathrm{s.t.} \, \, &\calL_{\bff} V(\bfx) + \calL_{\bfG} V(\bfx) \bfu + \alpha_l(V) \leq \delta \\
		&\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu \geq -\alpha_h(h) 
	\end{aligned}
\end{equation}
%
We could also formulate an equivalent DCP as demonstrated in the following proposition:
\begin{proposition}\label{DCP: LBQ-Equi} The following DCP formulation is equivalent to system \eqref{dynamics: Sys_dynamics} with control input generated by the CLF-CBF-QP proposed in \eqref{controller: CLF-CBF-QP}:
	%
	\begin{subequations}
		\label{DCP: LBQ-form}
		\begin{align}
			\dot{\bfx} = \bff(\bfx) + &\bfG(\bfx)[- \mathcal{L}_{\bfG}V(\bfx)^{\top}\bar{u}_l + \mathcal{L}_{\bfG}h(\bfx)^{\top}\bar{u}_h], \ \forall \bfx \in \calD \nonumber \\
			\mathrm{s.t.} \, \,  0 \leq \bar{u}_l &\perp -\calL_{\bff} V(\bfx) - \alpha_l(V) - \mathcal{L}_{\bfG}V(\bfx) \mathcal{L}_{\bfG}h(\bfx)^{\top}\bar{u}_h  \nonumber \\
			&+ [\mathcal{L}_{\bfG}V(\bfx) \mathcal{L}_{\bfG}V(\bfx)^{\top} + \frac{1}{p}]\bar{u}_l  \geq 0, \label{DCP_LBQ: CLC} \\
			0 \leq \bar{u}_h &\perp \calL_{\bff} h(\bfx) + \alpha_h(h) - \mathcal{L}_{\bfG}h(\bfx) \mathcal{L}_{\bfG}V(\bfx)^{\top}\bar{u}_l \nonumber \\
			&+ \mathcal{L}_{\bfG}h(\bfx) \mathcal{L}_{\bfG}h(\bfx)^{\top}\bar{u}_h \geq 0 \label{DCP_LBQ: CBC}
		\end{align}
	\end{subequations}
	%
	\begin{proof}
		The proof follows by evaluating the KKT conditions of CLF-CBF-QP \eqref{controller: CLF-CBF-QP}. First we obtain the close form expression of $\bfu$ w.r.t. Lagrangian multipliers $\lambda_1, \lambda_2$ by solving $\frac{\partial \calL}{\partial \bfu} = 0$, then we obtain the close form expression of $\delta$ w.r.t. Lagrangian multiplier $\lambda_1$ by solving $\frac{\partial \calL}{\partial \delta} = 0$. Substituting them into complementary constraints and the results follows. Note that in \eqref{DCP: LBQ-form} we use $\bar{u}_l$ and $\bar{u}_h$ to denote Lagrangian multipliers $\lambda_1$ and $\lambda_2$ respectively.
	\end{proof}
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%End of Appendix%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we justify our conclusion of DCP could achieve equivalency to QP based method through Proposition~\ref{DCP: BQ-Equi}, \ref{DCP: LBQ-Equi}. In the following section, we focus on the CBF-DCP formulation and demonstrate that how to choose a $\bfw_h$ other than the \textit{naive choice} to fully exploit the power of our formulation.
%\YY{Equivalency means same control input, revise later.}
%
\subsection{Choice of Design Parameters}
We have shown that our DCP framework could attain equivalency to QP based methods, as a result, local equilibria introduced in CBF-DCP \eqref{DCP: BQ-form} satisfies conditions proposed in Proposition \ref{prop: local_equi}. To remove these undesired local equilibria, instead of using our \textit{naive choice} of $\bfw_l$ and $\bfw_h$, we make the following modification: 
%
\begin{equation}
	\label{sel: bfw}
	\bfw_l = -\mathcal{L}_{\bfG}V(\bfx)^{\top}, \quad \bfw_h = \mathcal{L}_{\bfG}h(\bfx)^{\top} + k \bfw_p(\bfx)
\end{equation}
%
where $\bfw_p(\bfx)$ is locally Lipschitz and satisfies $\mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_p(\bfx) = 0, \bfw_p(\bfx) \neq \mathbf{0} \ \forall \bfx \in \calD$ with $k \in \bbR$. Apparently, CLF constraint \eqref{DCP: CLC} stays unchanged with $\bfw_l$ from \eqref{sel: bfw} comparing to our \textit{naive choice}. However, to make sure that $\bfw_p(\bfx) \neq \mathbf{0}$ while satisfying $\mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_p(\bfx) = 0$, we need to have $\mathcal{L}_{\bfG}h(\bfx) \in \bbR^m$ with $m \geq 2$, indicating that $\mathcal{L}_{\bfG}h(\bfx)$ is not a scalar. Thus we make the following assumption:

\begin{assumption}
	In addition to locally Lipschitz, $\bfG(\bfx)$ in \eqref{dynamics: Sys_dynamics} has full column rank with at least two columns.
\end{assumption}

Before demonstrating how to remove local equilibria characterized in (Proposition~\ref{prop: local_equi}) by selecting $k$, we want to show that our selection of $\bfw_h$ in \eqref{sel: bfw} will not change the solution of \eqref{DCP: CBC}. Substitute $\bfw_h = \mathcal{L}_{\bfG}h(\bfx)^{\top} + \bfw_p(\bfx)$ in \eqref{DCP: CBC} and we will have: $0 \leq \bar{u}_h \perp \bfF_h(\bfx) - \mathcal{L}_{\bfG}h(\bfx) \cdot \mathcal{L}_{\bfG}V(\bfx)^{\top}\bar{u}_l + \| \mathcal{L}_{\bfG}h(\bfx)^{\top} \|_2^2 \bar{u}_h + \mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_p(\bfx) k \bar{u}_h \geq 0$, however, $\mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_p(\bfx) = 0$ by assumption, so the CBF constraint \eqref{DCP: CBC} stays unchanged comparing to our \textit{naive choice} of $\bfw_h$. We introduce the following definition exploiting our findings above:
%
\begin{definition}[Unforced Dynamics]
	We define the unforced part of system \eqref{DCP: BQ-form} as follows:
	%
	\begin{equation}
		\label{dynamics: Unforced}
		\bfF_u(\bfx) = \bff(\bfx) + \bfG(\bfx)[-\mathcal{L}_{\bfG}V^{\top}\bar{u}_l +  \mathcal{L}_{\bfG}h^{\top} \bar{u}_h],
	\end{equation}
	%\SK{What is the definition of $\bar{\bfx}$? The equation \eqref{dynamics: Sys_unforced} is not really a system because both the trajectories of $\bar \bfx$ and $\bfx$ are not determined by \eqref{dynamics: Sys_unforced}. Following the derivation later, maybe just defining this as another function like $\bfF*(\bfx)$ and replacing $\bar \bfx$ in the latter equations would be good. }
	%
	with $\bar{u}_l = (f_l(\bfx))_+ = ( \frac{\mathcal{L}_{\bff}V + \alpha_l(V)}{\| \mathcal{L}_{\bfG}V \|_2^2} )_+$ and $\bar{u}_h = (f_h(\bfx))_+ = (-\frac{\mathcal{L}_{\bff}h - \mathcal{L}_{\bfG}h \cdot \mathcal{L}_{\bfG}V^{\top}\bar{u}_l }{\| \mathcal{L}_{\bfG}h \|_2^2})_+$.
\end{definition}	
%
\begin{remark}
Note that our selection of $\bfw_h$ will not introduce any extra local equilibria expect those on $\partial \calC$. One should notice that the constraint on $\bfw_p$ implies $\bfG(\bfx)\bfw_p \in \mathrm{null}(\nabla h(\bfx))$ and we have $\alpha_h(h) > 0, \forall \bfx \in \textrm{Int}(\calC)$ which ensures that $\bfF_u(\bfx) \notin \mathrm{null}(\nabla h(\bfx)), \forall \bfx \in \textrm{Int}(\calC): \bar{u}_h > 0$, as a result, we will not have $-\bfF_u(\bfx^*) = \bar{u}_h k \bfG(\bfx^*) \bfw_p$ in this case. And we could consult Proposition~\ref{prop: local_equi} directly for the case with $\bar{u}_h = 0$.
\end{remark}
%\begin{remark} By using $\bfw_h$ from \eqref{sel: bfw} we could represent every vectors satisfies $\mathcal{L}_{\bfG}h(\bfx) \cdot \bfw_h > 0$ and yield distinct $\bfw_h\bar{u}_h$. Since $\bfw_p(\bfx)$ could be any vector that belongs to the null space of $\mathcal{L}_{\bfG}h(\bfx)$ and any scaling term of $\mathcal{L}_{\bfG}h(\bfx)^{\top}$ will be compensated by $\bar{u}_h$.
%\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Section%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Local Equilibria Analysis}
From now on, we consider the CBF-DCP formulation \eqref{DCP: BQ-form} and use $\bfw_l, \ \bfw_h$ given in \eqref{sel: bfw}. To ease notation, we suppress the dependency on $\bfx$ of terms with Lie derivative and $\bfw_p$ in this section.

We have the close-loop system for our DCP formulation with $\bfw_l$ and $\bfw_h$ given by \eqref{sel: bfw} as follows: $\dot{\bfx} = \bfF_u(\bfx) + \bar{u}_h k \bfG(\bfx) \bfw_p$. Since we assume $\bfG(\bfx)$ to have full column rank, so we have: $\bfG(\bfx) \bfw_p \neq \mathbf{0}, \ \forall \bfx \in \partial \calD$. Also, as we pointed our in previous section, local equilibria will only be introduced on $\partial \calC$. Thus, if we have the following equation holds:
\begin{equation} \label{criteria: LE}
	-\bfF_u(\bfx^*) = \bar{u}_h k \bfG(\bfx^*) \bfw_p, \ \bfx^* \in \partial \calC
\end{equation}
then local equilibria exists. Now the problem becomes to find a $k$ with given a $\bfw_p$ such that \eqref{criteria: LE} does not hold on the boundary of the obstacle.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Forcing Term as a Modification to CBC Control Input}\label{k: constant}
First of all, one should notice that the constraint on $\bfw_p$ implies $\bfG(\bfx)\bfw_p \in \mathrm{null}(\nabla h(\bfx))$ and we also have $\bfF_u(\bfx) \in \mathrm{null}(\nabla h(\bfx)), \forall \bfx \in \partial \calC: f_h(\bfx) \geq 0$. Also, we must have $\bfF_u(\bfx)$ and $\bfG(\bfx) \bfw_p$ linearly dependent to make \eqref{criteria: LE} holds, as a result, if the given locally Lipschitz $\bfw_p$ satisfies $\| \bfF_u(\bfx) \|_2 \| \bfG(\bfx)\bfw_p \|_2- |\bfF_u(\bfx)^{\top}\bfG(\bfx)\bfw_p| > 0, \forall \bfx \in \partial \calC: \bar{u}_h > 0, \bfF_u(\bfx) \neq \mathbf{0}$, then every local equilibria will be removed and we could choose any constant $k \neq 0$.

Now considering the case where we have $\| \bfF_u(\bfx) \|_2 \| \bfG(\bfx)\bfw_p \|_2 + \bfF_u(\bfx)^{\top}\bfG(\bfx)\bfw_p = 0, \exists \bfx \in \partial \calC: \bar{u}_h > 0, \bfF_u(\bfx) \neq \mathbf{0}$, if we could find a finite constant $k$ such that:
%
\begin{equation}
	\label{criteria: k}
	k > \frac{\sup_{\bfx \in \calX_i} \| \bfF_u(\bfx) \|}{ \inf_{\bfx \in \calX_i} \bar{u}_h \| \bfG(\bfx) \bfw_p \|}
\end{equation}
%
with $\calX_i \coloneqq \{ \bfx \in \partial \calC: \| \bfF_u(\bfx) \|_2 \| \bfG(\bfx)\bfw_p \|_2 + \bfF_u(\bfx)^{\top}\bfG(\bfx)\bfw_p = 0, \bar{u}_h > 0, \bfF_u(\bfx) \neq \mathbf{0} \}$, then we will have every local equilibria removed. 

However, such a $k$ is not always available. If we have $\inf_{\bfx \in \calX_i} \bar{u}_h = 0$, then as a result $k$ will be infinite, nevertheless, we can conclude that the infimum is attained at some $\bfx_i \in \calS_i$ with $\calS_i \coloneqq \{ \bfx \in \partial \calC: \| \bfF_u(\bfx) \|_2 \| \bfG(\bfx)\bfw_p \|_2 + \bfF_u(\bfx)^{\top}\bfG(\bfx)\bfw_p = 0, f_h(\bfx) = 0, \bfF_u(\bfx) \neq \mathbf{0}, \calB_{\epsilon}(\bfx) \cap \calX_i \neq \emptyset, \forall \epsilon > 0 \}$ where $\calB_{\epsilon}(\bfx_c)$ denotes an abstract ball centered at $\bfx_c$ with radius $\epsilon$, in other words, $\calB_{\epsilon}(\bfx_c) \coloneqq \{ \bfx \in \bbR^n: \| \bfx - \bfx_c \|_2 \leq \epsilon \}$. 
\TODO{In that case, since a finite $k$ is no longer available through \eqref{criteria: k}, we use the following criteria instead:
%
\begin{equation}
	\label{criteria: relax_k}
	k > \frac{\sup_{\bfx \in \calX_i} \| \bfF_u(\bfx) \|}{ \nu \inf_{\bfx \in \calX_i} \| \bfG(\bfx) \bfw_p \|}
\end{equation}
%
where $\nu$ is a user-specific constant. Using such a $k$, local equilibria $\bfx^*$ only exists in the following set: $\calQ \coloneqq \{ \bfx \in \partial \calC: \| \bfF_u(\bfx) \|_2 \| \bfG(\bfx)\bfw_p \|_2 + \bfF_u(\bfx)^{\top}\bfG(\bfx)\bfw_p = 0, \bfF_u(\bfx) \neq \mathbf{0}, 0< \bar{u}_h \leq \nu \}$ satisfying $\bar{u}_h^*(\bfx^*) = \| \bfF_u(\bfx^*) \| / \| k \bfG(\bfx^*) \bfw_p \| $. One might find that by decreasing $\nu$, we will have $\calQ$ shrinking to $\calS_i$ and local equilibria $\bfx^*$ converging to corresponding $\bfx^*_i \in \calS_i$. 
%satisfying $\calB_{\epsilon}(\bfx^*_s) \cap \calX_i \neq \emptyset$ for arbitrary small $\epsilon > 0$. 
Thus, even though we still run into some local equilibria introduced by the extra forcing term, we could push them arbitrary close to their corresponding $\bfx^*_i$ by decreasing $\nu$. 

Although in this case (\eqref{criteria: k} yield infinite $k$) our approach will always admits some equilibria in set $\calQ$, we could make $\calQ$ shrinking to $\calS_i$. And if the trajectory of our system \eqref{DCP: BQ-form} will not run into $\calQ$, then it will not becomes an issue, so the question is under what conditions, the trajectory of \eqref{DCP: BQ-form} will run into $\calQ$. To better analysis this scenario, we first make an extra assumption on $f_h(\bfx)$:

\begin{assumption}
The partial derivative of $f_h(\bfx)$ with respect to $\bfx$: $\nabla f_h(\bfx)^{\top} = \partial f_h(\bfx) / \partial \bfx$ exists and locally Lipschitz at least on $\partial \calC$.
\end{assumption}

Based on the assumption above, we introduce the following definition:
%
\begin{definition}[Inseparable Points]
	We consider points on the boundary of our obstacle where $f_h(\bfx) = 0$ and the vector field generated by our system \eqref{dynamics: Sys_dynamics} is pointing to the non-decreasing direction of $f_h(\bfx)$. We denote the collection of such points as  $\bar{\calI}$ defined below:
	\begin{equation}
		\label{criteria: inse_points}
		\bar{\calI} \coloneqq \{ \bfx \in \partial \calC: \nabla f_h(\bfx) \bfF_u(\bfx) \geq 0, f_h(\bfx) = 0 \}.
	\end{equation}
\end{definition}
%
Since we could make $\calQ$ shrinking to $\calS_i$, so there might be an issue only if we wish to drive the trajectory of \eqref{DCP: BQ-form} towards $\calS_i$, by \textit{drive towards $\calS_i$} we mean: let $\calW \subset \partial \calC$ be a small neighborhood of $\calS_i$ such that $\nabla f_h(\bfx)^{\top} \bfG(\bfx)\bfw_p < 0, \| \bfF_u(\bfx) \|_2 \| \bfG(\bfx)\bfw_p \|_2- |\bfF_u(\bfx)^{\top}\bfG(\bfx)\bfw_p| = 0, f_h(\bfx) > 0, \bfF_u(\bfx) \neq \mathbf{0}$ for all $\bfx \in \calW$ and $\calW \cap \calQ \subseteqq \calW$. However, if we are driving the trajectory of \eqref{DCP: BQ-form} towards $\calS_i \setminus \bar{\calI}$, then we must have $\nabla f_h(\bfx) \bfF_u(\bfx) < 0$ for all $\bfx \in \calS_i \setminus \bar{\calI}$, indicating that there exists a small neighborhood $\calV$ of $\calS_i \setminus \bar{\calI}$ such that $\nabla f_h(\bfx) \bfF_u(\bfx) < 0, \forall \bfx \in \calV$, as a result, we have $\| \bfF_u(\bfx) \|_2 \| \bfG(\bfx)\bfw_p \|_2- \bfF_u(\bfx)^{\top}\bfG(\bfx)\bfw_p = 0, \forall \bfx \in \calV \cap \calW$, showing that $\bfF_u(\bfx)$ and $\bfG(\bfx)\bfw_p$ are in the same direction, which contradicts the definition of $\calS_i$ since there exists an $\epsilon^*$ such that $\calB_{\epsilon^*}(\bfx) \cap \calV \subseteq \calV, \forall \bfx \in \calS_i \setminus \bar{\calI}$ and we will have $\calB_{\epsilon^*}(\bfx) \cap \calX_i = \emptyset, \forall \bfx \in \calS_i \setminus \bar{\calI}$. So, we will have non-removable $\calQ$ on the trajectory of \eqref{DCP: BQ-form} only if we wish to drive our system towards $\calS_i \cap \bar{\calI}$.

To sum up, although our CBF-DCP always admits some local equilibria inside $\calQ$, we have a chance to remove them from the trajectory of our system by decreasing $\nu$ to make $\calQ$ shrinking towards $\calS_i$ unless we wish to drive our system to the following set: $\calS_i \cap \bar{\calI}$. But that will not hurt the stability of our system since we could not separate from $\partial \calC$ at those points belongs to $\calS_i \cap \bar{\calI}$ anyway. 
}
Moreover, if there exists a closed set defined as follows:
%
\begin{align}
	\calT := \{ \bfx \in \partial \calC | f_h(\bfx) \geq 0\}, \\
	\partial \calT := \{ \bfx \in \partial \calC | f_h(\bfx) = 0\}, \\
	\textrm{Int}(\calT) :=  \{ \bfx \in \partial \calC | f_h(\bfx) > 0\}.
\end{align} 
with $\partial \calT \subseteq \bar{\calI}$. Then our CBF-DCP formulation \eqref{DCP: BQ-form} renders $\calT$ forward invariant. As a result, once we enters $\calT$, we will never leave it and not to mention $\partial \calC$.
\YY{Need to revise some of the results in this subsection.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Forcing Term as a Permanent Control Input}\label{k: functional}
This method is to make $k$ as a function of $\bar{u}_h$ and takes the following structure: $k = \frac{k'}{\bar{u}_h}$, then we have the $\bar{u}_h k \bfG(\bfx) \bfw_p$ term equals to $k'\bfG(\bfx) \bfw_p$ and independent of $\bar{u}_h$. As a result, by using this method, the system dynamics has been changed and we should consider the following system:
%
\begin{equation}
	\label{dynamics: Forced_sys}
	\dot{\bfx} = \bff'(\bfx) + \bfG(\bfx)\bfu
\end{equation}
%
with $\bff'(\bfx) = \bff(\bfx) + k'\bfG(\bfx) \bfw_p$. 
And we modify the original DCP formulation accordingly:
%
\begin{subequations}
	\label{DCP: forced-form}
	\begin{align}
		&\dot{\bfx} = \bff'(\bfx) + \bfG(\bfx)[\bfw_l\bar{u}'_l + \bfw_h\bar{u}'_h], \ \forall \bfx \in \calD \nonumber \\
		\mathrm{s.t.} \, \, & 0 \leq \bar{u}'_l \perp -\bfF'_V(\bfx) - \mathcal{L}_{\bfG}V \cdot \bfw_l\bar{u}'_l \geq 0, \label{DCP_forced: CLC} \\
		& 0 \leq \bar{u}'_h \perp \bfF_h(\bfx) + \mathcal{L}_{\bfG}h \cdot [\bfw_l\bar{u}'_l + \bfw_h\bar{u}'_h] \geq 0 \label{DCP_forced: CBC}
	\end{align}
\end{subequations}
%
where $\bfw_l = -\mathcal{L}_{\bfG}V^{\top}, \bfw_h = \mathcal{L}_{\bfG}h^{\top}$ and $\bfF'_V(\bfx) = \mathcal{L}_{\bff'}V + \alpha_l(V)$. Notice that we have $\mathcal{L}_{\bff'}h = \nabla h \cdot [\bff(\bfx) + k'\bfG(\bfx) \bfw_p] = \nabla h \cdot \bff(\bfx) = \mathcal{L}_{\bff}h$ due to the fact that $\mathcal{L}_{\bfG}h \cdot \bfw_p = 0$, as a result we have $\bfF_h(\bfx)$ unchanged comparing to \eqref{DCP: BQ-form}.
According to Proposition~\ref{prop: local_equi}, our DCP system \eqref{DCP: forced-form} only admits local equilibria on the boundary of the obstacle with CBC constraint \eqref{DCP_forced: CBC} active. Hence we consider the following two cases:

\textbf{Case 1.} CLC constraint \eqref{DCP_forced: CLC} inactive: In this case, if we have:
%
\begin{equation}
	\label{le_forced_sys: clc_i}
	\mathbf{0} = \bff'(\bfx) + \bfG(\bfx)\bfw_h\bar{u}'_h
\end{equation}
%
where $\bar{u}'_h$ is given by solving \eqref{DCP_forced: CBC}: $\bar{u}'_h = -\frac{\mathcal{L}_{\bff}h}{\| \mathcal{L}_{\bfG}h \|^2_2}$, then local equilibria exists. Substituting $\bff'(\bfx)$ and $\bar{u}'_h$ into equation above and we have:
%
\begin{equation}
	\label{le_forced_sol: clc_i}
	k'\bfG(\bfx) \bfw_p = \frac{\mathcal{L}_{\bff}h}{\| \mathcal{L}_{\bfG}h \|^2_2} \bfG(\bfx)\mathcal{L}_{\bfG}h^{\top} - \bff(\bfx).
\end{equation}
%
Define:
%
\begin{equation}
	N_1 \coloneqq \sup_{\bfx \in \calU^i_{\calC}} \| \bfg_i(\bfx) \|, \ N_2 \coloneqq \inf_{\bfx \in \calU^i_{\calC}} \| \bfG(\bfx) \bfw_p \| \notag
\end{equation}
%
with $\calU^i_{\calC} \coloneqq \{ \bfx \in \partial \calC: \bar{u}'_h > 0, \bar{u}'_l = 0, \bfg_i(\bfx) \neq \mathbf{0}, \| \bfg_i(\bfx) \|_2 \| \bfG(\bfx) \bfw_p \|_2 + \bfg_i(\bfx)^{\top} \bfG(\bfx) \bfw_p = 0 \}$ and $\bfg_i(\bfx) = \bff(\bfx) + \bar{u}'_h \bfG(\bfx) \mathcal{L}_{\bfG}h^{\top}$.

\textbf{Case 2.} CLC constraint \eqref{DCP_forced: CLC} active: In this case, if we have:
%
\begin{equation}
	\label{le_forced_sys: clc_a}
	\mathbf{0} = \bff'(\bfx) + \bfG(\bfx)[\bfw_l\bar{u}'_l + \bfw_h\bar{u}'_h],
\end{equation}
%
where $\bar{u}'_l$ is given by solving \eqref{DCP_forced: CLC}: $\bar{u}'_l = \frac{\mathcal{L}_{\bff'}V + \alpha_l(V)}{\| \mathcal{L}_{\bfG}V \|_2^2} = f_l(\bfx) + k'\frac{\calL_{\bfG}V\bfw_p}{\| \mathcal{L}_{\bfG}V \|_2^2}$ and $\bar{u}'_h$ is given by solving \eqref{DCP_forced: CBC}: $\bar{u}'_h = -\frac{\mathcal{L}_{\bff}h - \mathcal{L}_{\bfG}h \mathcal{L}_{\bfG}V^{\top} \bar{u}'_l }{ \| \mathcal{L}_{\bfG}h \|_2^2 } = f'_h(\bfx) + k'\frac{\mathcal{L}_{\bfG}h \mathcal{L}_{\bfG}V^{\top} \mathcal{L}_{\bfG}V}{\| \mathcal{L}_{\bfG}h \|^2_2 \| \mathcal{L}_{\bfG}V \|_2^2}\bfw_p$, then local equilibria exists.
Substituting $\bff'(\bfx)$ and $\bar{u}'_l, \bar{u}'_h$ into equation above and we have:
%
%\begin{equation}
	%\label{le_forced_sol: clc_a}
	%\begin{aligned}
		%&\bff(\bfx) + k'\bfG(\bfx) \bfw_p - \frac{\mathcal{L}_{\bff}h}{\| \mathcal{L}_{\bfG}h 	%\|_2^2}\bfG(\bfx)\mathcal{L}_{\bfG}h^{\top} = \\
		%&\bar{u}'_l \bfG(\bfx) [\mathcal{L}_{\bfG}V^{\top} - \frac{\mathcal{L}_{\bfG}h \mathcal{L}_{\bfG}V^{\top}}{\| %\mathcal{L}_{\bfG}h \|^2_2}\mathcal{L}_{\bfG}h^{\top}].
	%\end{aligned}
%\end{equation}
%
%In order to separate $k'$, we rewrite equation above as:
%
\small
\begin{equation}
	\label{le_forced_sol: k'}
	\begin{aligned}
		&k'\bfG(\bfx) \bfw_p -  k'\frac{\calL_{\bfG}V\bfw_p}{\| \mathcal{L}_{\bfG}V \|_2^2} \bfG(\bfx) [\mathcal{L}_{\bfG}V^{\top} - \frac{\mathcal{L}_{\bfG}h \mathcal{L}_{\bfG}V^{\top}}{\| \mathcal{L}_{\bfG}h \|^2_2}\mathcal{L}_{\bfG}h^{\top}] = \\
		&k'\bfG(\bfx)[ \bfI_{m \times m} - \frac{\calL_{\bfG}V^{\top} \mathcal{L}_{\bfG}V}{\| \mathcal{L}_{\bfG}V \|_2^2} + \frac{\mathcal{L}_{\bfG}h^{\top} \mathcal{L}_{\bfG}h \mathcal{L}_{\bfG}V^{\top} \mathcal{L}_{\bfG}V}{\| \mathcal{L}_{\bfG}h \|^2_2 \| \mathcal{L}_{\bfG}V \|_2^2} ]\bfw_p = \\
		&k'\bfG(\bfx)\bfK(\bfx)\bfw_p = -\bff(\bfx) + \bfG(\bfx) [f_l(\bfx) \mathcal{L}_{\bfG}V^{\top} - f'_h(\bfx) \mathcal{L}_{\bfG}h^{\top}]
	\end{aligned}
\end{equation}
\normalsize
%
Define:
%
\begin{equation}
	N_3 \coloneqq \sup_{\bfx \in \calU^a_{\calC}} \| \bfg_a(\bfx) \|, \ N_4 \coloneqq \inf_{\bfx \in \calU^a_{\calC}} \| \bfG(\bfx) \bfK(\bfx) \bfw_p \| \notag,
\end{equation}
%
with $\calU^a_{\calC} \coloneqq \{ \bfx \in \partial \calC: \bar{u}'_h > 0, \bar{u}'_l > 0, \bfg_a(\bfx) \neq \mathbf{0}, \| \bfg_a(\bfx) \|_2 \| \bfG(\bfx) \bfK(\bfx) \bfw_p \|_2 + \bfg_a(\bfx)^{\top} \bfG(\bfx) \bfK(\bfx) \bfw_p = 0 \}$ and $\bfg_a(\bfx) = \bff(\bfx) + \bfG(\bfx) [-f_l(\bfx) \mathcal{L}_{\bfG}V^{\top} + f'_h(\bfx) \mathcal{L}_{\bfG}h^{\top}]$. 

If we could find a finite constant $k' > \max(\frac{N_1}{N_2}, \frac{N_3}{N_4})$ then we will have every local equilibria removed. However, such $k'$ is not always available since $N_4$ could be zero. Due to the assumption that $\bfG(\bfx)$ has full column rank, $N_4 = 0 \iff \bfK(\bfx) \bfw_p = \mathbf{0}, \bfx \in \calU^a_{\calC}$. We consult the following proposition to determine the conditions under which $\bfK(\bfx) \bfw_p$ would be zero.
\begin{proposition}
	Consider non-zero vectors $\bfa, \bfb \in \bbR^{m \times 1}$ with $m \geq 2$ and $\bfc \in \textit{null}(\bfb)$. The following equation holds 
	\begin{equation}
		[\bfI_{m \times m} - \frac{\bfa\bfa^{\top}}{\bfa^{\top}\bfa} + \frac{\bfb\bfb^{\top}\bfa\bfa^{\top}}{\bfb^{\top}\bfb\bfa^{\top}\bfa}]\bfc = \mathbf{0}
	\end{equation}
	if and only if we have $\bfa$ and $\bfc$ linearly dependent. 
	\begin{proof}
		We could write $\bfa$ in the following form: $\bfa = a\bfb + \sum_{i = 1}^{m-1}b_i\bfb_i^{\perp}$ where $\bfb_i^{\perp}$ forms an orthonormal basis of the null space of $\bfb$ and with out loss of generality, we assume $\bfc = \bfb_k^{\perp}$. Now we have: $\frac{\bfb\bfb^{\top}\bfa\bfa^{\top}}{\bfb^{\top}\bfb\bfa^{\top}\bfa} = a \frac{\bfb\bfa^{\top}}{\bfa^{\top}\bfa}$ and $\bfa^{\top}\bfc = b_k$. As a result we have the following equation:
		$(a^2 \| \bfb \|_2^2 + \sum_{i = 1}^{m-1}b_i^2) \bfb_k^{\perp} - b_k\bfa + ab_k\bfb = (a^2 \| \bfb \|_2^2 + \sum_{i = 1}^{k-1}b_i^2 + \sum_{j = k + 1}^{m-1}b_j^2) \bfb_k^{\perp} - b_k(\sum_{i = 1}^{k-1}b_i\bfb_i^{\perp} + \sum_{j = k + 1}^{m-1}b_j\bfb_j^{\perp}) = \mathbf{0}$. Since we need to have at least one $a, b_i \neq 0$, the only solution to the equation above is $a = 0$ and $b_i = 0, \ \forall i \neq k$. Thus the result follows.
	\end{proof}
\end{proposition}
So, if we could find a locally Lipschitz $\bfw_p$ such that $\mathcal{L}_{\bfG}V^{\top}$ and $\bfw_p$ are linearly independent for all $\bfx \in \calU^a_{\calC}$, then we could find a finite constant $k'$ such that $k' > \max(\frac{N_1}{N_2}, \frac{N_3}{N_4})$. And as a result, our DCP system \eqref{DCP: forced-form} admits no local equilibria with such $k'$.
\begin{remark}
	One should notice that in \eqref{DCP: forced-form} the extra forcing term $\bfG(\bfx)\bfw_p$ appears in our system dynamics as a permanent control input and as a result, the original drift term $\bff(\bfx)$ has been changed to $\bff'(\bfx)$. So, one should not use this method if the original drift term is of particular interest.
\end{remark}
\YY{Compare two different approaches, answer the question: what kind of local equilibria we can't remove. Based on the simulation results, I think we could remove subsection B since it does not have a very good result.}


==> tex/Old_background.tex <==

\NA{Add references to Pol and Jorge, Dimos Dimarogonas, Dimitra Panagou, Michael Posa}
\section{Preliminaries}
In this section, we give a brief overview of control Lyapunov functions, control barrier functions and introduce the notion of safe set $\calC$. We show that the CBF-QP method will introduce local equilibria on the boundary of the safe set. We also introduce the definition of index-zero affine DCP and provide conditions on the existence and uniqueness of its solution which will serve as the foundation of our CBF-DCP controller.
\subsection{System Dynamics, CLF and CBF}
Consider the following nonlinear control affine system:
%
\begin{equation}
	\label{dynamics: Sys_dynamics}
	\dot{\bfx} = \bff(\bfx) + \bfG(\bfx)\bfu
\end{equation}
%
with the state variable $\bfx \in \calX \subseteq \bbR^n$ and the control input $ \bfu \in \bbR^m$, where $\bff : \bbR^n \to \bbR^n$ and $\bfG : \bbR^n \to \bbR^{n \times m}$ are locally Lipschitz. A typical task of the control problem is to design a stabilizing controller. The stability of the system is often shown by a Lyapunov function, and the control design is derived by considering the control Lyapunov function defined below.
%
%\SK{I would add another sentence like "A typical task of the control problem is to design a stabilizing controller. The stability of the system is often shown by a Lyapunov function, and the control design is derived by considering the control Lyapunov function defined below." } 
%
\begin{definition}[CLF] \label{CLF}
	A positive definite function V: $\calX \to \bbR$ is a control Lyapunov function (CLF) for system \eqref{dynamics: Sys_dynamics} if there exists a control input $\bfu$ such that:
	%
	\begin{equation} \label{criteria: CLF}
		\inf_{\bfu \in \bbR^m} [ \calL_{\bff} V(\bfx) + \calL_{\bfG} V(\bfx) \bfu ] \leq -\alpha_l(V), \ \forall \bfx \in \calX
	\end{equation}
	%
	where $\alpha_l: \bbR_{\geq 0} \to \bbR_{\geq 0}$ is a class $\calK$ function \cite{khalil1996nonlinear}.
\end{definition}
%
With $V$ a valid CLF, the corresponding stabilizing control set is: 
%
\begin{equation}
	\nonumber
	K_{clf}(\bfx) = \{ \bfu \in \bbR^m: \calL_{\bff} V(\bfx) + \calL_{\bfG} V(\bfx) \bfu \leq -\alpha_l(V) \}.
\end{equation}
%
In the context of safety, we consider a set $\calC$ defined as the zero-superlevel set of a continuously differentiable function $h: \calD \subseteq \calX \to \bbR$, yielding:
%
\begin{align}
	\calC := \{ \bfx \in \calD | h(\bfx) \geq 0\}, \\
	\partial \calC := \{ \bfx \in \calD | h(\bfx) = 0\}, \\
	\textrm{Int}(\calC) :=  \{ \bfx \in \calD | h(\bfx) > 0\}.
\end{align} 
%
where $\partial \calC$ and $\textrm{Int}(\calC)$ denotes boundary and interior of set $\calC$ respectively.
The set $\calC$ is referred as the safe set based on the following definition.
%
\begin{definition} [Safety] 
	The system in \eqref{dynamics: Sys_dynamics} is safe with respect to set $\calC$ defined above if $\calC$ is forward invariant, i.e., for every $\bfx_0 \in \calC$, $\bfx(t) \in \calC$ for all $t \in I(\bfx_0)$, where $I(\bfx_0)$ is a maximum interval of existence such that $\bfx(t)$ is the unique solution to \eqref{dynamics: Sys_dynamics} on $I(\bfx_0)$ \cite{ames2017clfcbfqp}. 
\end{definition} 
%
In order to guarantee safety, forward invariant of set $\calC$ is desired, which is shown by the non-negativeness of a barrier function, and the control design is derived by considering the control barrier function defined below.
%
\begin{definition}[CBF]\label{CBF}
	A continuously differentiable function $h(\bfx): \calD \to \bbR$ is a control barrier function (CBF) for system \eqref{dynamics: Sys_dynamics} with respect to $\calC$ if there exists a control input $\bfu$ such that:
	%
	\begin{equation} \label{criteria: CBF}
		\sup_{\bfu \in \bbR^m} [ \calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu ] \geq -\alpha_h(h), \forall \bfx \in \calD
	\end{equation}
	%
	where $\alpha_h: \bbR \to \bbR$ is an extended class $\calK$ function \cite{ames2019cbf}.
\end{definition}
%
With $h$ a valid CBF, the corresponding safe control set is: 
%
\begin{equation}
	\nonumber
	K_{cbf}(\bfx) = \{ \bfu \in \bbR^m: \calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu \geq -\alpha_h(h) \}.
\end{equation}
%
\subsection{CBF-QP Introduce Local Equilibria}
For safety critical systems, finding a single control input $\bfu$ achieving both stability and safety is sometimes infeasible. In order to guarantee safety when \eqref{criteria: CLF} and \eqref{criteria: CBF} are not compatible, a popular approach is to have the CLF constraint automatically relaxed when CBF constraint is active, which leads to the CBF-QP method defined as follows \cite{ames2019cbf}:
%
\begin{equation}\label{controller: CBF-QP}
	\begin{aligned}
		\bfu(\bfx) = & \argmin_{\bfu \in \bbR^m} || \bfu - \bfr(\bfx) ||_2^2  \\
		&\mathrm{s.t.} \, \, \calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu \geq -\alpha_h(h)
	\end{aligned}
\end{equation}
%
where $\bfr(\bfx) \in K_{clf}$ and locally Lipschitz.
Suppose following assumptions holds throughout this paper:
%
\begin{assumption}
	There exists a CBF $h: \calD \to \bbR$ for system \eqref{dynamics: Sys_dynamics} with $\mathbf{0} \in \calC$ and $\calD$ an open set. Also, $\calL_{\bfG} h(\bfx) \neq \mathbf{0}, \forall \bfx \in \calD$.
\end{assumption}
%
\begin{assumption}
	There exists a CLF $V: \calX \to \bbR$ for system \eqref{dynamics: Sys_dynamics} with $\bff(\mathbf{0}) + \bfG(\mathbf{0})\bfr(\mathbf{0}) = \mathbf{0}, \bfr(\bfx) \in K_{clf}$. Also, $\calL_{\bfG} V(\bfx) \neq \mathbf{0}, \forall \bfx \in \calX$.
\end{assumption}
%
We could obtain the close-form solution of \eqref{controller: CBF-QP} as follows through KKT conditions:
%
\begin{proposition}\label{sol: QP}
	Consider system \eqref{dynamics: Sys_dynamics} with $\nabla h(\bfx) ^{\top} = \partial h / \partial \bfx$ and $\bfe(\bfx) = \bff(\bfx) + \bfG(\bfx)\bfr(\bfx)$. For all $\bfx_0 \in \calC$, the solution to \eqref{controller: CBF-QP}  is given by \cite{ames2014acc}, \cite[Theorem 1]{shaw2022croa}:
	\begin{equation}\label{sol: CBF-QP}
		\bfu^*(\bfx) = \left\{
		\begin{aligned}
			&\bfr(\bfx), \ &\nabla h(\bfx) \cdot \ \bfe(\bfx) + \alpha_h(h) \geq 0, \\
			&\bar{\bfu}(\bfx), \ &\nabla h(\bfx) \cdot \bfe(\bfx) + \alpha_h(h) < 0,
		\end{aligned} \right.
	\end{equation}
	where 
	\begin{equation}\nonumber
		\bar{\bfu}(\bfx) = \bfr(\bfx) - \frac{\nabla h(\bfx) \cdot \ \bfe(\bfx) + \alpha_h(h)}{\| \calL_{\bfG} h(\bfx) \|_2^2} \calL_{\bfG} h(\bfx)^{\top}.
	\end{equation}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Appendix%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%\begin{proof}
		%The Lagrangian associated to \eqref{controller: CBF-QP} is given by:
		%\begin{equation}
			%\label{deriv: Lagran}
			%\begin{aligned}
			%	\calL &= \frac{1}{2} || \bfu - \bfr(\bfx) ||_2^2 \\
			%	&- \lambda( \calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu + \alpha_h(h) )
			%\end{aligned}
		%\end{equation}
		%and the KKT conditions are:
		%\begin{subequations}
			%\begin{align}
			%	\frac{\partial \calL}{\partial \bfu} =  \bfu - \bfr(\bfx) - \lambda \calL_{\bfG} h(\bfx)^{\top} &= 0 \label{deriv: partial} \\
			%	\lambda( \calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu + \alpha_h(h) ) &= 0 \label{deriv: complem}
			%%\end{subequations}
		%with $\lambda \geq 0$. At this point, we have two different scenarios: \par
		%\textbf{Case 1:} In this case, we have $\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu + \alpha_h(h) > 0$, so that $\lambda = 0$. According to \eqref{deriv: partial}, we have $\bfu = \bfr(\bfx)$. As a result, when $\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfr(\bfx) + \alpha_h(h) > 0$ holds, we have $\bfu = \bfr(\bfx)$.
  
		%\textbf{Case 2:} In this case, we have $\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) \bfu + \alpha_h(h) = 0$, so that $\lambda \geq 0$. According to \eqref{deriv: partial}, we have $\bfu = \bfr(\bfx) + \lambda \calL_{\bfG} h(\bfx)^{\top}$. $\lambda$ is obtained by solving: $\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx) ( \bfr(\bfx) + \lambda \calL_{\bfG} h(\bfx)^{\top} ) + \alpha_h(h) = 0$. As a result, we have:
		%\begin{equation}
			%\nonumber
			%%\lambda = -\frac{\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx)\bfr(\bfx) + \alpha_h(h)}{\| \calL_{\bfG} h(\bfx) \|_2^2}.
		%\end{equation}
		%Note that in this case we require $\lambda \geq 0$ so we need to have $\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx)\bfr(\bfx) + \alpha_h(h) \leq 0$. However, if the inequality above holds with equality, we end up with $\lambda = 0$, which admits: $\bfu = \bfr(\bfx)$. \par
		%Above all, $\bfu$ is given by the following equation:
		%\begin{equation}\nonumber
			%\bfu^*(\bfx) = \left\{
			%\begin{aligned}
			%	&\bfr(\bfx), \ &\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx)\bfr(\bfx) + \alpha_h(h) > 0, \\
			%	&\bfr(\bfx), \ &\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx)\bfr(\bfx) + \alpha_h(h) = 0, \\
			%	&\bar{\bfu}(\bfx), \ &\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx)\bfr(\bfx) + \alpha_h(h) < 0,
			%\end{aligned} \right.
		%\end{equation}
		%with $\bar{\bfu}(\bfx) = \bfr(\bfx) - \frac{\calL_{\bff} h(\bfx) + \calL_{\bfG} h(\bfx)\bfr(\bfx) + \alpha_h(h)}{\| \calL_{\bfG} h(\bfx) \|_2^2} \calL_{\bfG} h(\bfx)^{\top}$.
	%\end{proof}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%End of Appendix%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{proposition}
%
Although \eqref{controller: CBF-QP} ensures safety for system \eqref{dynamics: Sys_dynamics}, stability is still a concern. Actually, QP-based methods like \eqref{controller: CBF-QP} are known to introduce local equilibria other than the origin \cite{reis2020control}. Those local equiilibria are characterized by the following proposition.
\begin{proposition} \label{prop: local_equi}
	For close-loop system $\dot{\bfx} = \bff(\bfx) + \bfG(\bfx)\bfu^*$ with $\bfu^*$ given in \eqref{sol: CBF-QP}, local equilibria $\bfx^*$ only exists on $\partial \calC$ and satisfies:
	\small
	\begin{equation}\label{criteria: LE-QP}
		\bff(\bfx^*) = - \bfG(\bfx^*)\bfr(\bfx^*) + \frac{\nabla h(\bfx^*) \cdot \ \bfe(\bfx^*)}{\| \calL_{\bfG} h(\bfx^*) \|_2^2} \bfG(\bfx^*) \calL_{\bfG} h(\bfx^*)^{\top}
	\end{equation}
	\normalsize
	and $\nabla h(\bfx^*) \cdot \ \bfe(\bfx^*) < 0$.
	\begin{proof}
		One should notice that $\nabla h(\bfx^*) \cdot \ \bfe(\bfx^*) < 0$ indicating that the CBF constraint is active on the boundary of the obstacle, so we begin our proof by showing that local equilibria only exists when CBF constraint is active, i.e., $\nabla h(\bfx) \cdot \bfe(\bfx) + \alpha_h(h) < 0$. When CBF constraint is inactive, we have $\bfu = \bfr(\bfx)$ and close-loop system $\dot{\bfx} = \bfe(\bfx)$ satisfying $\nabla V(\bfx) \cdot \bfe(\bfx) \leq -\alpha_l(V)$ with $\nabla V ^{\top}(\bfx) = \partial V / \partial \bfx$. Since we have $\alpha_l(V) \neq 0, \forall \bfx \in \calC \setminus \{ \mathbf{0} \}$, indicating that $\nabla V(\bfx) \neq \mathbf{0}$ and $\bfe(\bfx) \neq \mathbf{0}, \forall \bfx \in \calC \setminus \{ \mathbf{0} \}$, which concludes the first part of our proof. Now considering the case when CBF constraint is active, according to KKT conditions, we require $\nabla h(\bfx) \cdot \dot{\bfx} + \alpha_h(h) = 0$. It is easy to notice that $\nabla h(\bfx) \neq \mathbf{0}$ and $\dot{\bfx} \neq \mathbf{0}, \forall \bfx \in \calC \setminus \partial \calC$, due to the fact that $\alpha_h(h) \neq 0, \forall \bfx \in \textrm{Int}(\calC)$. As a result, local equilibria could only be introduced when $\alpha_h(h) = 0$, which implies that $\bfx \in \partial \calC$ and \eqref{criteria: LE-QP} comes from $\dot{\bfx} = \bff(\bfx) + \bfG(\bfx)\bar{\bfu} = \mathbf{0}$.
	\end{proof}
\end{proposition}
%
%\SK{I would recommend defining the local equilibria as $\bfx^*$ and showing \eqref{criteria: LE-QP} with replacing $\bfx$ by $\bfx^*$. }
%
\subsection{Index-Zero DCP}
In this section we introduce a special class of index-zero differential complementary probelm (DCP) and provide existence and uniqueness conditions for its solution. 

\TODO{Content in Parts with Issue section should be here.}

%\YY{Introduce P-matrix before this proposition.}
In the following sections, we tackle the following problems:



\begin{problem}[Stabilizing Safe Control] \label{prob: safe control}
    Design a control input $\bfu$ for control-affine system \eqref{dynamics: Sys_dynamics} so that the closed-loop system becomes asymptotically stable at the origin and safe with respect to the set $\calC$.
\end{problem}

\begin{problem}[Local Equilibria Characterization] \label{prob: local equi}
    Determine sufficient conditions on the existence of local equilibria for control-affine system \eqref{dynamics: Sys_dynamics} with $\bfu$ derived in Problem~\ref{prob: safe control}.
\end{problem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%TEMP%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%We tackle the following problems. 
%
%\begin{prob}[Stabilizing Safe Control]
%Design a control input $\bfu$ for control-affine system \eqref{eq: Sys} so that the closed-loop system becomes %asymptotically stable at the origin and safe with respect to the set $\calC$.
%\end{prob}

%Our proposed stabilizing safe control is demonstrated in autonomous navigation scenario, where a CBF function is constructed %online using surface point measurements of the obstacles, such as those provided by a Lidar scanner.
%\NA{We can remove the second problem since we do not really have a very new or different idea to solve it. Instead, add discussion explaining that our safe stabilizing controller is demonstrated in autonomous navigation simulations, where a CBF function is constructed online using surface point measurements of the obstacles, such as those provided by a Lidar scanner.}


%\begin{prob}[CBF Approximation]
%For some unknown obstacles, given a data set $\calD = \{ \bfp_i \}_{i = 1}^N %$ containing position information of surface points of the obstacles, obtain %an approximated CBF $\hat{h}(\bfx)$.
%\end{prob}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tex/Old_intro.tex <==
\section{Introduction} 
Safety and stability are key properties in shared-autonomy to avoid undesired scenarios, such as collisions among autonomous robots and humans, operating in the same environment. Satisfying both safety and stability requires adaptation of the automated robot based on the action and information of the human through interaction, which needs to be accounted in the control design.
%\NA{How does the interaction influence the CBF or CLF design?}  
In the community of control systems and robotics, the safety constraints are often represented by Control Barrier Function (CBF), while the stabilization objective is often described by a Control Lyapunov Function (CLF). 
%On the other hand, \NA{The workshop is about human-robot interaction and shared autonomy. We need to write the paper in a way that connects to the theme. I suggest reading the abstract here \url{https://sites.google.com/view/saphri-icra2022/home?authuser=0} and trying to use some of its keywords in the motivation and introduction for our paper.}. A crucial aspect of successfully deploying such systems is satisfaction of safety constraints and stability objectives, which are often represented by Control Barrier Functions (CBFs) and Control Lyapunov Functions (CLFs). 
A pioneering work on CBF-based control design \cite{ames2017clfcbfqp} unifies CBFs with CLFs as constraints in a quadratic program (QP). The CLF-CBF-QP approach which has been successfully applied to a variety of systems, such as walking robots \cite{ahmadi2020risk} and adaptive cruse control \cite{ames2014acc}. 

%%%%%%%%%%%%
A differential complementarity problem combines an ordinary differential equation with complementarity constraints, which provides a powerful modeling paradigm for system in which discontinuities are present.
%\NA{You may skip the discussion of index one. We do not explain it anywhere in the draft.}
%In this paper, we consider an index one DCP since the uniqueness 
We propose a novel formulation of safe and stable control synthesis as an index zero DCP \cite{pang2008dvi}. 
%\NA{Introduce the DCP problem first. What is it? Why do we consider it? What is the importance of index one?}. 
%%%%%%%%%%%%
%Unlike the CBF-CLF-QP method in \cite{ames2017clfcbfqp}, where control barrier constraints are derived based on set invariant theory to ensure safety, in the proposed method we solve an index one DCP associated with a hyper-parameter $\lambda$. The hyper-parameter is set to zero when the system is operating in its safe state, making the system follows its stabilizing trajectory. On the other hand, when the system needs to get around an obstacle due to zero CBF, the DCP solution yields a non-zero hyper-parameter $\lambda$, making the system travel along the zero level set of the CBF. 

==> tex/bogdan-old.tex <==
Let $\sigma_1(\bfy)\ge...\ge \sigma_n(\bfy)$ denote the singular values of $\bfA(y)$. If $\bfA(\bfy)$, $\bfq(\bfy)$ are Lipschitz continuous functions of $\bfy$ and there exists $\sigma>0$, such that $\sigma_n(\bfy) >\sigma$, $\forall \bfy$, then $\bfC(\bfy, \bfz) = \bfA(y)\bfz +\bfq(\bfz)$ is Lipschitz continuous in $\bfy$ and strongly monotone in $\bfz$ and thus the DCP \eqref{criteria: index-zero_DCP} is equivalent to a Lipschitz ODE.

In order to obtain the existence and uniqueness result for DCP \eqref{criteria: index-zero_DCP}, we need to define the notions of stability and strong stability of LCP solutions. 
\begin{definition}[LCP solution stability, \cite{PangLCP}]
Let $\bfq \in \R^n$ and $\bfA\in \R^{n \times n}$ be given. Let 
$\mathrm{SOL}(\bfq, \bfA)$ denote the solution set of $\mathrm{LCP}(\bfq,\bfA)$. A solution $\bfz^*$ of $\mathrm{LCP}(\bfq,\bfA)$ is said to be {\bf stable} if there are neigborhoods $V$ of $\bfz^*$ and $U$ of the pair $(\bfq,\bfA)$ such that 
\begin{enumerate}
    \item[(i)] $\forall\; (\overline{\bfq}, \overline{\bfA}) \in U $, the set 
    $$
       S_V(\overline{\bfq}, \overline{\bfA}) = \mathrm{SOL}(\overline{\bfq}, \overline{\bfA}) \cap V
    $$
    is non-empty.
    \item[(ii)] $\sup \{ ||\bfy -\bfz^*||:\; \bfy \in S_V(\overline{\bfq}, \overline{\bfA})\} \to 0$ as 
    $(\overline{\bfq}, \overline{\bfA})$ approaches $(\bfq, \bfA)$.
\end{enumerate}
The solution $\bfz^*$ is called {\bf strongly stable} if $S_V(\overline{\bfq}, \overline{\bfA})$ is a singleton.
\end{definition}


To obtain an existence and uniqueness result for the DCP \eqref{criteria: index-zero_DCP}, we combine the $P$-matrix assumption on the matrix $\bfA(\bfy)$ with the  strong stability assumption on the solution of $\mathrm{LCP}(\bfq(\bfy), \bfA(\bfy))$. These assumptions must hold uniformly with respect to $\bfy$

==> tex/waste.tex <==
\section{Parts With Issue}
\subsection{An Index-Zero DCP}
{\color{cyan} We consider the following dynamical system under complementary constraints
\begin{equation}\label{criteria: index-zero_DCP}
		\begin{aligned}
			& \dot{\bfy} = \bfF(\bfy,\bfz) \\
			\mathrm{s.t.} \, \, & 0 \leq \bfz \perp \bfA(\bfy) \bfz + \bfq(\bfy) \geq 0,
		\end{aligned}
	\end{equation}
	where the $\bfa \perp \bfb$ sign means that $\bfa$ and $\bfb$ are orthogonal as vectors, in other words $\bfa^{\top} \bfb = 0$.
The dynamical system \eqref{criteria: index-zero_DCP} is also known as a differential complementarity problem (DCP). We say that this DCP has index $0$ if we can show that it  is  equivalent to a system of ordinary differential equations. This can be done if the  complementarity  constraint uniquely determines $z$ as a function of $y$.
}
\begin{comment}
\begin{definition}[Index-Zero DCP]\label{DCP}
	Considering the following dynamical system under complementary constraint:
	\begin{equation}\label{criteria: index-zero_DCP}
		\begin{aligned}
			& \dot{\bfy} = \bfF(\bfy,\bfz) \\
			\mathrm{s.t.} \, \, & 0 \leq \bfz \perp \bfA(\bfy) \bfz + \bfq(\bfy) \geq 0,
		\end{aligned}
	\end{equation}
	where the $\bfa \perp \bfb$ sign means that $\bfa$ and $\bfb$ are orthogonal as vectors, in other words $\bfa^{\top} \bfb = 0$.
	\begin{equation}\label{criteria: index-zero_DCP}
		\begin{aligned}
			& \dot{\bfy} = \bfF(\bfy,\bfz) \\
			\mathrm{s.t.} \, \, & 0 \leq \bfz \perp \bfA(\bfy) \bfz + \bfq(\bfy) \geq 0,
		\end{aligned}
	\end{equation}
	where the $\bfa \perp \bfb$ sign means that $\bfa$ and $\bfb$ are orthogonal as vectors, in other words $\bfa^{\top} \bfb = 0$. \SK{The current statement doesn't give any definition. Maybe we should add a sentence "The system \eqref{criteria: index-zero_DCP} is DCP with index-zero."?}\NA{Refer to \url{http://www2.mathematik.hu-berlin.de/~iccp-2014/dl/slides/ICCP2014_David_Stewart_Slides.pdf} for a concise explanation.}
\end{definition}
\end{comment}

{\color{cyan} The next result shows that under certain assumptions on the matrix $\bfA(\bfy)$ the DCP has index $0$ and a locally unique solution exists.
\begin{comment}
An existence and uniqueness  result for the DCP above can be obtained if the underlying matrix is a $P$--matrix. 
\end{comment}
We first recall the notion of a $P$-matrix in the definition below.
	\begin{definition}[P-matrix, \cite{PangLCP}]
		A matrix $\bfA\in \mathbb{R}^{m\times m}$ is said to be a $P$-matrix if all its principal minors are positive.
	\end{definition}
}

The solution of \eqref{criteria: index-zero_DCP} is {\color{blue}characterized} by the following proposition:
\begin{proposition} \label{prop: DCP_uniqueness}
	%	If we have the determinants of all of the  principle sub-matrices of $\bfA(\bfy)$ are positive for all $\bfy$, then $\bfA(\bfy)$ is a P-matrix and the solution of \eqref{criteria: index-zero_DCP} is unique \cite{shen2005linear}.
	If the matrix $\bfA(\bfy)$ is a $P$-matrix $\forall \bfy$, then the DCP \eqref{criteria: index-zero_DCP} has index $0$ and a locally unique solution exists,  \cite{shen2005linear,PangLCP}.
	
	
\end{proposition}
